Historia: Refuting Callback Reachability with Message-History Logics (Extended Version)

This paper determines if a callback can be called by an event-driven framework in an unexpected state.Event-driven programming frameworks are pervasive for creating user-interactive apps on just about every modern platform.Control flow between callbacks is determined by the framework and largely opaque to the programmer.This opacity of the callback control flow not only causes difficulty for the programmer but is also difficult for those developing static analysis.Previous static analysis techniques address this opacity either by assuming an arbitrary framework implementation or attempting to eagerly specify all possible callback control flow, but this is either too coarse or too burdensome and tricky to get right.Instead, we present a middle way where the callback control flow can be gradually refined in a targeted manner to prove assertions of interest.The key insight to get this middle way is by reasoning about the history of method invocations at the boundary between app and framework code - enabling a decoupling of the specification of callback control flow from the analysis of app code.We call the sequence of such boundary-method invocations message histories and develop message-history logics to do this reasoning.In particular, we define the notion of an application-only transition system with boundary transitions, a message-history program logic for programs with such transitions, and a temporal specification logic for capturing callback control flow in a targeted and compositional manner.Then to utilize the logics in a goal-directed verifier, we define a way to combine after-the-fact an assertion about message histories with a specification of callback control flow.We implemented a prototype message history-based verifier called Historia that enables proving the absence of multi-callback bug patterns in real-world open-source Android apps.

==> Makefile <==
######################################################################
# Makefile
#
# Makefile for LaTeX projects
######################################################################

BASE = main
PAPERS = $(BASE)

# Generate short bib
# -e 's/^[ 	]*[Dd]oi/OPTdoi/' \ # removed because it breaks things
%.short.bib: %.orig.bib
	sed -e 's/@string{SHORT/@string{/' \
            -e 's/^[ 	]*[Ee]ditor/OPTeditor/' \
            -e 's/^[ 	]*[Mm]onth/OPTmonth/' \
            -e 's/^[ 	]*[Pp]ublisher/OPTpublisher/' \
            -e 's/^[ 	]*[Aa]ddress/OPTaddress/' \
            -e 's/^[ 	]*[Ii]sbn/OPTisbn/' \
            -e 's/^[ 	]*[Ii]ssn/OPTissn/' \
            -e 's/^[ 	]*[Uu]rl/OPTurl/' \
            -e 's/^[ 	]*[Pp]ages/OPTpages/' \
            -e 's/^[ 	]*[Cc]rossref/OPTcrossref/' \
            -e 's/^[ 	]*[Ss]eries/OPTseries/' \
            $< > $@
						
include bectex.mk


==> bectex/Makefile <==
######################################################################
# Makefile
#
# Makefile for LaTeX projects
######################################################################

BASE = main
PAPERS = $(BASE)

# Generate short bib
%.short.bib: %.orig.bib
	sed -e 's/@string{SHORT/@string{/' \
            -e 's/^[ 	]*[Ee]ditor/OPTeditor/' \
            -e 's/^[ 	]*[Mm]onth/OPTmonth/' \
            -e 's/^[ 	]*[Pp]ublisher/OPTpublisher/' \
            -e 's/^[ 	]*[Aa]ddress/OPTaddress/' \
            -e 's/^[ 	]*[Ii]sbn/OPTisbn/' \
            -e 's/^[ 	]*[Ii]ssn/OPTissn/' \
            -e 's/^[ 	]*[Uu]rl/OPTurl/' \
            -e 's/^[ 	]*[Dd]oi/OPTdoi/' \
            -e 's/^[ 	]*[Pp]ages/OPTpages/' \
            -e 's/^[ 	]*[Cc]rossref/OPTcrossref/' \
            -e 's/^[ 	]*[Ss]eries/OPTseries/' \
            $< > $@
						
include bectex.mk


==> decision-procedure.tex <==
\section{Encoding Message History Judgments as Temporal Formula}
\label{sec:decision}

\JEDI{Automated reasoning about abstract message histories and \newls by giving procedures for 3 judgments}
In this section, we show our syntax-directed encoding of abstract message histories and specifications into temporal formula.
Such an encoding enables automation of proofs over the judgments
used in \autoref{sec:applog}, namely, unsatisfiability ($\feasible{\abstrace}$), excludes initial ($\notinit{\abstrace}$), and
entailment ($\entail{\abstrace}{\abstrace'}$).
The high level intuition is that each of these judgments can be encoded such that they may be dispatched to a SMT solver by first encoding from abstract message histories to temporal formula and finally encoding to first order logic.
The reasoning over abstract message histories here may be extended to the full abstract program state $\abspstate$ using techniques presented in prior work (for example \cite{berdine+2005:symbolic-execution} and \cite{DBLP:conf/cav/PiskacWZ13} present automated approaches to reasoning about separation logic).
% Each of these judgments may be encoded as a satisfiability check over temporal formula that can be decided by a SMT solver as we showed in Section \ref{sec:decidable}.

\JEDI{target of this section is to show soundness of our encoding}
The goal of this section is to give a sound encoding of each judgment such that unsatisfiability of a SMT call means the judgment holds.
Theorems \ref{thm:contradiction}, \ref{thm:excludes}, and \ref{thm:entail} define soundness for each judgment and follow from the definition of concretization section \ref{sec:applog}. 
Intuitively, unsatisfiability checks if no history, $\hist$, can satisfy the abstract message history $\abstrace$.
Excludes-initial takes an abstract message history, $\abstrace$, and proves that the empty history, $\histemp$, is not in the concretization.  
Entailment, $\entail{\abstrace}{\abstrace'}$, proves that every concrete state in the first abstract state, $\abstrace$, is contained in the second, $\abstrace'$.

\begin{theorem}[Sound Unsatisfiability]
	If $\feasible{\abstrace}$ then $\withvalua{\hist} \not\models_{\SpecSet} \abstrace$ for all $\withvalua{\hist}$.
	\label{thm:contradiction}
\end{theorem}

\begin{theorem}[Sound Excludes-Initial]
	If $\notinit{\abstrace}$ then $\withvalua{\histemp} \not\models_{\SpecSet} \abstrace$ for all $\valua$.
	\label{thm:excludes}
\end{theorem}

\begin{theorem}[Sound Entailment]
	If $\entail{\abstrace}{\abstrace'}$ and $\inconc{\withvalua{\hist}}{\abstrace}$ then $\inconc{\withvalua{\hist}'}{\abstrace'}$ for some $\valua'$.
	\label{thm:entail}
\end{theorem}

% The process for reducing each of these judgments is split into two steps, first a reduction from a specification and abstract message history to a temporal formula, Figure \ref{fig:auxfun}, and then, a reduction from temporal formula to first order logic, Figure \ref{fig:redFol}.

\JEDI{Each judgment can be defined based on an encoding relation and unsat call.}
% The primary challenge of computing judgments over abstract message histories is combining the meaning of an abstract message history, $\abstrace$, with the meaning of the provided specification, $\SpecSet$.
% For all three judgments, the abstract message history and specification are reduced into a single temporal formula. 
% This single formula is then easier to reason about than the combined semantics of the specification set and abstract message history.
\autoref{fig:atencode} defines the judgments for unsatisfiable excludes-init and entailment over abstract message histories.
Importantly, the premise of each judgment relies on a matching temporal formula judgment that does not take the specification, $\SpecSet$.
This is possible due to the temporal formula encoding, $\encodeRel{\abstrace}{\SpecSet}{\directive}$, discussed later.
Unsatisfiable holds over an abstract message history $\abstrace$ if it encodes to the temporal formula $\directive$ and the temporal formula is unsatisfiable via temp-unsatisfiable.
Excludes initial holds if the encoded abstract message history also excludes the initial message history via temp-excludes-initial.
Entailment encodes both abstract message histories and holds if the first encoding entails the second.
The corresponding judgments over temporal formula rely on calls to the SMT solver using uninterpreted first-order logic where interpretations for message history properties such as less than are axiomatized in the formula $\histAxiomsFol$.
A temporal formula is unsatisfiable, temp-unsatisfiable, if the first order logic encoding with the axioms discussed earlier is also unsatisfiable.
Temp-excludes-initial holds for an abstract message history if the first-order logic encoding is unsatisfiable with the additional axiom that the length of the message history is zero.
Entailment holds if a message history does not exist such that it is modeled by the premise abstract message history but not the consequent abstract message history.
The temp-excludes-initial judgment holds if a formula where the premise abstract message history is conjuncted with a negated encoding of the consequent abstract message history.
The axioms are only applied positively and not negated since they are shared between the premise and consequent.
Free variables in the consequent are universally quantified as the formula is negated, no variables should be shared between the premise formula and the consequent formula.


% \TODO{rm below}
% Judgments over the temporal formula may be decided by encoding the temporal formula to equivalent first-order logic formula that are unsatisfiable if the judgment holds.
% We explain how each judgment in \autoref{fig:atencode} and how it uses the encoding to temporal formula and then to first-order logic. To determine feasibility of an abstract trace, it is sufficient to show that the historic formula encoding cannot model any message histories.  
% Determining excludes initial, it is sufficient to show that the temporal formula encoding also excludes initial.
% Entailment may be determined if the temporal formula of the first state entails the temporal formula of the second.

% \TODO{following is stale, look at overview and update}
% This reduction step may be explained more clearly by examining one direction of the ``iff'' used to define concretization of abstract message histories: If $\inconc{\withvalua{\hist}}{\abstrace}$ and $\modDir{\withvalua{\msg}}{\absmsg}$ then $\inconc{\histcons{\hist}{\msg}}{\abstrace}$. Assuming that we have some message, $\msg$, concatenated to the abstract message history, $\hist$, the history must satisfy all history implications from the specification matching the message resulting in instantiation compilation step. Additionally, once such requirements have been instantiated, messages may affect temporal formula already instantiated resulting in the quotient compilation step.

% \TODO{(shawn) remove this paragraph if it remains in the overview}
% For example, we show the compilation of two states from Section \ref{sec:overview}, $\refstate{1}:\ronepre \abstracebase$ and $\abspstate_2:\rtwopre \ronepre \abstracebase$~from Section \ref{sec:overview} where \codej{unsubscribe} and \codej{call} must happen in the future. 
% When instantiating $\abspstate{1}$, \codej{call} is instantiated using Specification \ref{spec:call} and the instantiate judgment to $\exists \codej{s},\codej{t},\absof{f}. [ \niDir{\enkwCi~s.\codej{unsubscribe()}}{\enkwCi~s := \codej{t.subscribe(}\absof{f}\codej{)}} ]$ and then, when \codej{unsubscribe} is added for $\abspstate_2$, the quotient judgment gives us  
% $\exists \codej{s},\codej{t},\absof{f}.[ \niDir{\enkwCi~\codej{s.unsubscribe()}}{\enkwCi~\codej{s} := \codej{t.subscribe(}\absof{f}\codej{)}} ] \wedge \codej{s} \neq \absof{s}$, finally, it is encoded to first order logic.

\begin{figure}[b]
\begin{footnotesize}	
\begin{mathpar}
	\fbox{%
	$\feasible{\abstrace}$
	\\
	$\notinit{\abstrace}$
	\\
	$\entail{\abstrace}{\abstrace'}$
	}\\

	\infer[unsatisfiable]{
		\encodeRel{\abstrace}{\SpecSet}{\directive} \\ \dirEntailBot{\directive}
	}{
		\feasible{\abstrace}
	}

	\infer[excludes-initial]{
		\encodeRel{\abstrace}{\SpecSet}{\directive} \\ \empNotEntailDir{\directive}
		% \unsat{\exists \withvalua{\hist}. \hist = \histemp \wedge \toFOL{\atEncode{\abstrace}{\SpecSet}}}
	}{
		\notinit{\abstrace}
	}
	
	\infer[entailment]{
		\encodeRel{\abstrace}{\SpecSet}{\directive}\\
		\encodeRel{\abstrace'}{\SpecSet}{\directive'}\\
		\dirEntailDir{\directive}{\directive'}
	}{\entail{\abstrace}{\abstrace'}} \\

	\fbox{
		$\dirEntailBot{\directive}$ \\
		$\empNotEntailDir{\directive}$ \\
		$\dirEntailDir{\directive}{\directive'}$
	}\\
	
	\infer[temp-unsatisfiable]{
		\toFOLRel{\directive}{\fol} \\ \folEntailBot{\fol}
	}{
		\dirEntailBot{\directive}
	}

	\infer[temp-excludes-initial]{
		% 
		\toFOLRel{\directive}{\fol} \\ \empNotEntailFol{\fol}
	}{\empNotEntailDir{\directive}}

	\infer[temp-entailment]{
		\toFOLRel{\directive}{\fol} \\ \toFOLRel{\directive'}{\fol'} \\ \folEntailFol{\fol}{\fol'}
	}{
		\dirEntailDir{\directive}{\directive'}
	}	
\end{mathpar}
\end{footnotesize}
\Description{}
\caption{The unsatisfiable, excludes-initial, and entailment judgments over abstract message histories hold if the corresponding encoding of temporal formulas hold. 
%The reduction from decisions over temporal formula, i.e. $\dirEntailBot{\directive}$, $\empNotEntailDir{\directive}$, and $\dirEntailDir{\directive}{\directive'}$, are defined in figure \ref{fig:redFol}.
Judgments over temporal formula use the first order logic encoding and a call to a SMT solver with $\unsat{}$. 
A conjunction of axioms, $\histAxiomsFol$, from Section \ref{sec:decidable} model interpreted properties in the uninterpreted first order logic such as a total order on message indices.
}
\label{fig:auxfun}
\end{figure}

\JEDI{encoding of abs msg hist equiv to abs msg hist as long as history is realizable in msg history}
The key to the soundness of the encoding is showing a relation between abstract message histories specifications and temporal formula, $\encodeRel{\abstrace}{\SpecSet}{\directive}$, such that the realizable histories (i.e. $\hist \models \SpecSet$) that satisfy $\abstrace$ also satisfy $\directive$. 
We first utilize Lemma \ref{lem:encode} to prove the use of the encoding relation and, later, we explain the encoding relation in detail.

%\TODO{prove by induction on encoding derivation}
%\TODO{omega models s in consequent of first part of lemma 5.4 should be removed, can assume from omega models abst hist.}
\begin{lemma}[correct encode]
%$\inconc{\withvalua{\hist}}{\abstrace}$ if and only if $\encodeRel{\abstrace}{\SpecSet}{\directive}$, $\modeldouble{\hist}{\valua} \models \directive$, and $\hist \models \SpecSet$ for all $\withvalua{\hist}$.
\hspace{\linewidth}
\begin{enumerate}
\item For all abstract messages $\absmsg$ and assignments $\valua$, there exists a (concrete) message $\msg$ such that $\inconc{\withvalua{\msg}}{\absmsg}$.\TODO{Move this into the body text, probably}
\item \label{lem:encodefwd} If $\encodeRel{\abstrace}{\SpecSet}{\directive}$ and $\inconc{\withvalua{\hist}}{\abstrace}$ then $\modeldouble{\hist}{\valua} \models \directive$.
\item \label{lem:encodebkg} If $\encodeRel{\abstrace}{\SpecSet}{\directive}$ and $\modeldouble{\hist}{\valua} \models \directive$ and $\hist \models \SpecSet$ then $\inconc{\withvalua{\hist}}{\abstrace}$.
\end{enumerate}
\label{lem:encode}
\end{lemma}

\JEDI{Proof of sound unsat and excludes initial}
Proving unsatisfiability sound is straightforward, due to lemma \ref{lem:encode} we can see that satisfiability the encoding of the abstract message history, $\withvalua{\hist}\models\directive$, is a necessary condition for the message history itself to be satisfiable.  Since we know the encoding $\directive$ is unsatisfiable from Corrolary \ref{lem:tempref}, we also know that the abstract message history is unsatisfiable.
Proving excludes initial is similar to unsatisfiability, the extra axiom that the length is zero makes Corollary \ref{lem:tempex} hold.

\JEDI{Proof of sound entailment}
The proof for entailment is slightly more complicated as we need to account for a negation.
From the premise of \thmref{entail} the encoding of $\abstrace$ and $\abstrace'$ are $\directive$ and $\directive'$, and we have that $\entail[]{\directive}{\directive'}$.
From $\entail[]{\directive}{\directive'}$ and Corollary \ref{lem:tempentail} we have that $\withvalua{\hist}\models \directive$ implies $\withvalua[\valua']{\hist}\models \directive'$ for some $\valua'$.
%If $\withvalua{\hist}\models \directive$ implies $\withvalua[\valua']{\hist}\models \directive'$ for some $\valua'$, then $\withvalua{\hist}\models \directive$ and $\hist\models\SpecSet$ implies $\withvalua[\valua']{\hist}\models \directive'$ for some $\valua'$ and $\hist\models\SpecSet$.
The premise of \thmref{entail} gives us  $\inconc{\withvalua{\hist}}{\abstrace}$, Lemma \ref{lem:encode} gives us that $\hist\models\SpecSet$ and $\withvalua{\hist} \models \directive$.
With the other direction of \thmref{entail}, we know that $\hist\models\SpecSet$ and $\withvalua{\hist} \models \directive$ and have proved entailment.


The following corollaries can be seen from \thmref{tempFolEq} and the judgments in \autoref{fig:auxfun} as the temporal formula encoding in first order logic is equisatisfiable.

\begin{corollary}[sound temp-refute]
If $\dirEntailBot{\directive}$ then $\notModDir{\withvalua{\hist}}{\directive}$ for all $\withvalua{\hist}$.
\label{lem:tempref}
\end{corollary}

\begin{corollary}[sound temp-excludes-initial]
If $\empNotEntailDir{\directive}$ then $\notModDir{\withvalua{\histemp}}{\directive}$ for all $\assignment$.
\label{lem:tempex}
\end{corollary}

\begin{corollary}[sound temp-entail]
If $\dirEntailDir{\directive}{\directive'}$ then $\modDir{\withvalua{\hist}}{\directive}$ implies $\modDir{\withvalua[\assignment']{\hist}}{ \directive'}$ for some $\assignment'$.
\label{lem:tempentail}
\end{corollary}

\JEDI{High level description of encoding relation}
\paragraph{Syntax directed encoding of abstract message histories as temporal formula.}
\autoref{fig:atencode} shows the syntax directed encoding introduced in \autoref{sec:overview}.
The encode judgment is inductively defined on the structure of the abstract message history, $\abstrace$.
Encode-okhist results in the formula true (we assume well formed message histories match the result).
Encode-next is inductive on the abstract message history and uses two additional judgment forms at each step, instantiate ($\instRel{\absmsg}{\SpecSet}{\directive}$) and quotient ($\updRel{\directive}{\directive'}{\absmsg}$).
Instantiate constrains a history based on a hypothesized next message and the effect of a history implication.
Quotient removes a message from the end of history implications instantiated in the ``future''.
Since the length of the history is unknown, the formula determining if a message history is realizable, $\hist \models \SpecSet$, is unbounded, the direct encoding to first order logic would also be unbounded (due to the conjunction over indices in Figure \ref{fig:cbcfsemantics}) therefore the base case is that $\abstracebase$ encodes to true. 


%By expanding the semantics of \newls from \autoref{fig:cbcfsemantics} we know that $\hist$ must match each $\directive$  $\withvalua{\histcons{\hist}{\msg}} \models \abstrace$ holds if $\hist \models \SpecSet$ and $\inconc{\withvalua{\histcons{\msg}{\hist}}}{\abstrace}$   \TODO{===} and apply Lemma \ref{lem:inst}


Lemma \ref{lem:encode} is proven by induction on the abstract trace, $\abstrace$, utilizing Lemmas \ref{lem:inst} and \ref{lem:quot}.  The proof is listed in Appendix \ref{sec:atencproof}. 
Briefly, the base case holds due to the definition of $\abstracebase$ and the inductive case, $\abstracecons{\absmsg}{\abstrace}$, holds because of the two auxiliary functions: 
\begin{inparaenum}
\item $\instRel{\absmsg}{\SpecSet}{\directive}$ precisely capture the constraints on messages modeled by$\abstracecons{\absmsg}{\abstrace}$ from rules matching $\absmsg$ (\autoref{lem:inst}), and % the encoding captures temporal formula from rules that match $\absmsg$
\item $\updRel{\directive}{\absmsg}{\directive'}$ precisely removes $\absmsg$ from the end of each trace modeled by $\directive$ (\autoref{lem:quot}).
\end{inparaenum}

\begin{figure}\small
  \begin{mathpar}
    \fbox{$\encodeRel{\abstrace}{\SpecSet}{\directive}$

      $\instRel{\absmsg}{\SpecSet}{\directive}$

      $\updRel{\directive}{\directive'}{\absmsg}$}\\

    %\infer[encode-okhist]{ }{
    \infer{ }{
      \encodeRel{\abstracebase}{\SpecSet}{\text{true}}
    }

    %\infer[encode-next]{
    \infer{
      \instRel{\absmsg_1}{\SpecSet}{\directive_1'} \\
      \encodeRel{\abstrace_2}{\SpecSet}{\directive_2} \\
      \updRel{\directive_2}{\directive_2'}{\absmsg_1}
    }{
      \encodeRel{\abstracecons{\abstrace_2}{\absmsg_1}}{\SpecSet}{ \directive_1' \wedge \directive_2'}
    }\\

    %\infer[instantiate-message-equal]{
    \infer{
      %\SpecSet = \specOnly{\absmsg_2}{\directive} \\
      \ideq{\absmsg_1}{\absmsg_2} %\\ \instRel{\absmsg_1}{\SpecSet'}{\directive'}
    }{
      \instRel{\absmsg_1}{(\specOnly{\absmsg_2}{\directive})}{
        %\directive[\fv{\absmsg_1} / \fv{\absmsg_2}]
        [\unifysubst]\directive
      }
    }

    %\infer[instantiate-message-not-equal]{
    \infer{
      %\SpecSet = \specOnly{\absmsg_2}{\directive} \\
      \idneq{\absmsg_1}{\absmsg_2} %\\ \instRel{\absmsg_1}{\SpecSet'}{\directive}
    }{
      \instRel{\absmsg_1}{(\specOnly{\absmsg_2}{\directive})}{\text{true}}
    }\\
%    
    % \infer[instantiate-base]{ }{
    %   \instRel{\absmsg}{\text{true}}{\text{true}}
    % }
    % \\

    %\infer[quotient-once]{
    \infer{
      %\directive = (\msgnotequiv{\ltmsg}{\absmsg} \wedge \iDir{\ltmsg}) \vee \msgequiv{\ltmsg}{\absmsg}
    }{
      \updRel{\iDir{\ltmsg}}{
	\msgequiv{\ltmsg}{\absmsg} \vee
        (\msgnotequiv{\ltmsg}{\absmsg} \wedge \iDir{\ltmsg})
      }{\absmsg}
    }

    %\infer[quotient-has-not]{ }{
    \infer{ }{
      \updRel{\notiDir{\ltmsg}}{
	\notiDir{\ltmsg} \wedge \msgnotequiv{\ltmsg}{\absmsg}
      }{\absmsg}
    }

    %\infer[quotient-not-since]{
    \infer{
      %\directive = (\msgequiv{\ltmsg_2}{\absmsg} \vee (\msgnotequiv{\ltmsg_2}{\absmsg} \wedge \niDir{\ltmsg_1}{\ltmsg_2})) \wedge \msgnotequiv{\ltmsg_1}{\absmsg}
    }{
      \updRel{\niDir{\ltmsg_1}{\ltmsg_2}}{
        (\msgequiv{\ltmsg_2}{\absmsg} \vee (\msgnotequiv{\ltmsg_2}{\absmsg} \wedge \niDir{\ltmsg_1}{\ltmsg_2})) \wedge \msgnotequiv{\ltmsg_1}{\absmsg}
      }{\absmsg}
    }
%
    % \infer[quotient-and]{\updRel{\directive_1}{\directive_1'}{\absmsg} \\ \updRel{\directive_2}{\directive_2'}{\absmsg} }{
    %   \updRel{\directive_1 \wedge \directive_2}{\directive_1' \wedge \directive_2'}{\absmsg}
    % }
%
    % \infer[quotient-or]{\directive_1' = \updRel{\directive_1}{\directive_1'}{\absmsg} \\ \directive_2' = \updRel{\directive_2}{\directive_2'}{\absmsg} }{
    %   \updRel{\directive_1 \vee \directive_2}{\directive_1' \vee \directive_2'}{\absmsg}
    % }
%
    % \infer[quotient-eq]{ }{
    %   \updRel{\absof{x} = \absof{y}}{\absof{x} = \absof{y}}{\absmsg}
    % }
%
    % \infer[quotient-true]{ }{
    %   \updRel{\text{true}}{\text{true}}{\absmsg}
    % }
%
    % \infer[quotient-false]{ }{
    %   \updRel{\text{false}}{\text{false}}{\absmsg}
    % }
%    
    % \infer[quotient-forall]{\updRel{\directive}{\directive'}{\absmsg} }{
    %   \updRel{\forall\ \absof{x}.~\directive}{\forall\ \absof{x}.~\directive'}{\absmsg}
    % }
%
    % \infer[quotient-exists]{\updRel{\directive}{\directive'}{\absmsg} }{
    %   \updRel{\exists\ \absof{x}.~\directive}{\exists\ \absof{x}.~\directive'}{\absmsg}
    % }
  \end{mathpar}
	\caption{
		Encoding of abstract message histories and specifications to temporal formula which are equivalent under realizable message histories.
	}
	\label{fig:atencode}
\end{figure}

Now, we describe the compilation steps instantiate and quotient in more detail including their soundness.
Reasoning about the equivalence of abstract messages and weak abstract messages is needed for the auxiliary functions.  
We use $\msgequiv{\ltmsg}{\absmsg}$ to reduce the comparison of abstract messages to temporal formula.  
For messages with different names (e.g. \codej{call} and \codej{onCreate}) or for different kinds of messages (e.g. $\enkwCi$ vs $\enkwCb$), $\msgequiv{\ltmsg}{\absmsg}$ results in the temporal formula "false".
When the names and kind of message is the same, $\msgequiv{\ltmsg}{\absmsg}$ results in a conjunction comparing each non-quantified argument of $\ltmsg$ to the corresponding argument of $\absmsg$ (the parameter arity is the same if the names are the same).

The instantiate encoding step, $\instRel{\absmsg}{\SpecSet}{\directive}$ is correct as long as appending a message in $\absmsg$ to a message history modeled by $\directive$ is still modeled by the specification and removing a message $\msg$ from a message history $\histcons{\hist}{\msg}$ such that the message is in an abstract message history $\absmsg$ means that the history $\hist$ models $\directive$. 
% \begin{inparaenum}
% \item instantiating an abstract message $\absmsg$ means that any message and assignment that models the abstract message, $\withvalua{\msg}\models\absmsg$, appended on a realizable message history, $\histcons{\hist}{\hist}\models \SpecSet$, means that the history models the temporal formula, $\withvalua{\hist}\models\directive$  (Lemma \ref{lem:inst}), and 
% \item 
% \end{inparaenum}
Proof of Lemma \ref{lem:inst} follows from the semantics in \autoref{fig:cbcfsemantics}.
% For each history implication in the specification, either instantiate-message-equal or instantiate-message-not-equal applies resulting in a conjunction of requirements.
If a history implication may match the hypothesized message, instantiate-message-equal, the consequent of the history implication has the free variables of the abstract message swapped for the free variables of the target of the history implication, $\directive[\fv{\absmsg_1} / \fv{\absmsg_2}]$ (note that this substitution matches the corresponding arity of each abstract value in $\absmsg_1$ and $\absmsg_2$).
The free variables of the target message, $\absmsg_2$, are either a super set or equal to the free variables of the temporal formula, $\directive$.
Swapping the free variables corresponds to the semantics of temporal formula, Figure \ref{fig:cbcfsemantics}, since $\exists y. \forall x. x=y \Rightarrow \text{p}(x)$ is logically equivalent to $\exists y.  \text{p}(y)$. 
If a history implication does not match, instantiate-message-not-equal, then the consequent is true as the premise is false.

\begin{lemma}[correct instantiate]
	\hspace{\linewidth}
	\begin{enumerate} 
		\item \label{lem:instfwd} If $\histcons{\hist}{\msg} \models \SpecSet$ and $\modDir{\withvalua{\msg}}{\absmsg}$ and $\instRel{\absmsg}{\SpecSet}{\directive}$ then $\modDir{\withvalua{\hist}}{\directive}$.
		\item \label{lem:instbkg} If $\hist \models \SpecSet$ and $\modDir{\withvalua{\msg}}{\absmsg}$ and $\instRel{\absmsg}{\SpecSet}{\directive}$ and $\withvalua{\hist}\models\directive$ then $\histcons{\hist}{\msg} \models \SpecSet$.
		% \item If $\hist \models \SpecSet$ and $\modDir{\withvalua{\msg}}{\absmsg}$ and $\instRel{\absmsg}{\SpecSet}{\directive}$ then $\histcons{\hist}{\msg} \models \SpecSet$.
		%\item If $\histcons{\hist}{\msg} \models \SpecSet$ and $\modDir{\withvalua{\msg}}{\absmsg}$ and $\modDir{\withvalua{\hist}}{\directive}$ then $\instRel{\absmsg}{\SpecSet}{\directive}$. (TODO: wrong because a bad $\directive$ could be chosen)
	\end{enumerate}
	% $\histcons{\hist}{\msg} \models \SpecSet$ if and only if $\instRel{\absmsg}{\SpecSet}{\directive}$, $\modDir{\withvalua{\hist}}{\directive}$, and $\modSpec{\hist}{\SpecSet}$ for all $\msg$, $\assignment$, and $\hist$ such that $\modDir{\withvalua{\msg}}{\absmsg}$.
	% $\hist;\msg \models \SpecSet$ if and only if ($\hist \models \instEncode{\absmsg}{\SpecSet}$ and $\hist \models \SpecSet$) for all messages, $\msg$, in the abstract message, $\withvalua{\msg}\models\absmsg$.
	\label{lem:inst}
\end{lemma}
 
The quotient compilation step removes an abstract message from the end of each history captured by a temporal formula (as shown by Lemma \ref{lem:quot}). 
Figure \ref{fig:atencode} defines the quotient auxiliary function for each syntactic production in the abstract message history.
A quotient of a weak abstract message in a Once formula with an abstract message, $\updRel{\iDir{\ltmsg}}{\absmsg}{\directive}$, results in two possibilities for the temporal formula $\directive$. Either 
\begin{inparaenum}
	\item $\ltmsg$ is the same as $\absmsg$ releasing the once requirement, or
	\item $\ltmsg$ is different from $\absmsg$ and does not affect the once requirement.
\end{inparaenum}
For Not Since, $\updRel{\niDir{\ltmsg_1}{\ltmsg_2}}{\absmsg}{\directive}$, it must be the case that $\absmsg$ is different from $\ltmsg_1$ and then the same conditions for Once apply over $\ltmsg_2$.
Has Not, $\updRel{\notiDir{\ltmsg}}{\absmsg}{\directive}$, simply requires $\ltmsg$ to be different from $\absmsg$.
Quotient over true, false, and equality results in the same formula. The boolean operations, $\wedge$ and $\vee$ result in a quotient of each operand.

\begin{lemma}[correct quotient]
	\hspace{\linewidth}
	\begin{enumerate}
		\item \label{lem:quotfwd} If $\withvalua{\histcons{\hist}{\msg}}\models\directive$ and $\withvalua{\msg}\models\absmsg$ and $\updRel{\directive}{\directive'}{\absmsg}$ then $\withvalua{\hist}\models\directive'$.
		\item \label{lem:quotbkg} If $\withvalua{\hist}\models\directive'$ and $\withvalua{\msg}\models \absmsg$ and $\updRel{\directive}{\directive'}{\absmsg}$ then $\withvalua{\histcons{\hist}{\msg}}\models\directive$.
	\end{enumerate}
	\hspace{\linewidth}
	% $\updRel{\directive}{\directive'}{\absmsg}$ and $\modDir{\withvalua{\histcons{\hist}{\msg}}}{\directive}$ if and only if $\modDir{\withvalua{\hist}}{\directive'}$ for all  $\withvalua{\msg}$ such that $\modDir{\withvalua{\msg}}{\absmsg}$.
%$\withvaluaind{\hist}{\histlen{\hist}} \models \updEncode{\directive}{\absmsg}$ if and only if $\withvaluaind{\hist;\msg}{\histlen{\hist;\msg}} \models \directive$ for all messages, $\msg$ in the abstract message, $\withvalua{\msg}\models \absmsg$.
\label{lem:quot}
\end{lemma}

% \paragraph{Decidability of first-order logic encoding}

% The encodings of unsatisfiable ($\feasible{\abstrace}$) and
% exclude-initial ($\notinit{\abstrace}$) judgments described earlier do not introduce any quantifiers
% , $\encodeRel{\abstrace}{\SpecSet}{\directive}$.
% The resultant FOL formulas are still well-formed and therefore in EPR. Consequently, we have the following
% corollaries:
% \begin{corollary}[Unsatisfiable is decidable]
%   For any specification set $\SpecSet$ and abstract message history
%   $\abstrace$, the refutation judgment $\feasible{\abstrace}$ is
%   decidable.
% \end{corollary} 


% \begin{corollary}[Exclude-Initial is decidable]
%   For any specification set $\SpecSet$ and abstract message history
%   $\abstrace$, the exclude-initial judgment $\notinit{\abstrace}$ is
%   decidable.
% \end{corollary}

\paragraph{Consequences of Decidability}
Refutation and excludes initial over temporal formula are both decidable as the encoding 
is a conjunction of well formed temporal formula and quotienting adds no quantifiers.  
However, entailment is not within the decidable fragment due to the negation of the temporal formula encoding.
As a consequence of the extended EPR encoding of the abstract trace,
both unsatisfiable ($\feasible{\abstrace}$) and exclude-initial
($\notinit{\abstrace}$) judgments always terminate when the encoding is dispatched to a SMT
solver (As shown in the evaluation, section \ref{sec:eval}).
However, the FOL encoding of entailment
($\entail{\directive}{\directive'}$) judgment could not be proven decidable due to the negation of a first order formula.
% , i.e., 
% $\exists~\fv{\directive}.~\toFOL{\directive} \wedge \forall~\fv{\directive'}.~\neg\toFOL{\directive'}$, 
% could not be shown to be decidable, resulting in SMT solver timing out on complex entailment queries.


\iffalse
\TODO{Rewrite above this line -----------------------------}
\TODO{Find better way to express entailment as sub judgments, right now it would be a "for all" "exists" over assignments which doesn't seem great.}

 \TODO{finish expanding definitions, possibly add theta to decision judgments below}



The judgments are parameterized on the specification set, $\SpecSet$, which captures the
user's assumptions about the framework's behavior.  Concretely,
$\SpecSet$ is a collection of \newls rules, whose syntax is
described in Sec.~\ref{sec:newls}. Computing the aforementioned
judgments entails encoding the abstract message history, $\abstrace$,
as a first order logic (FOL) formula over a concrete message history,
$\omega$. The three judgments can then be cast as (un)satisfiability
checks on their FOL encodings.

The refutation judgment ($\feasible{\abstrace}$) is
valid if the FOL encoding of the abstract trace, i.e.,
$\exists \omega.  \toFOL{\atEncode{\abstrace}{\SpecSet}
}$, is unsatisfiable. The auxiliary function
$\atEncode{\cdot}{\SpecSet}$ takes an abstract trace, $\abstrace$, a
specification set, $\SpecSet$, and returns an ``extended'' consequent \TODO{get rid of ext consequent},
$\phidec$, which is simply the consequent ($\phi$) from
Fig.~\ref{fig:cftl} extended with conjunctions and existential
quantification:

Note that the consequent (extended or otherwise) is not yet a FOL
formula as it contains \newls combinators like $\mathbf{HN}$.
Compiling to $\phidec$ is an intermediary step in the multi-step
process of encoding to FOL, which is described below.

Like the refutation judgment, the excludes-initial and subsumption
judgments have equivalent FOL encodings. The judgment
$\notinit{\abstrace}$ is valid iff $\exists \omega. \omega = \epsilon
\wedge \toFOL{\atEncode{\abstrace}{\SpecSet}}$ is
unsatisfiable. Likewise the judgment
$\entail{\abstrace_1}{\abstrace_2}$ holds iff $\exists \omega.
\toFOL{\atEncode{\abstrace_1}{\SpecSet}} \wedge \neg
\toFOL{\atEncode{\abstrace_2}{\SpecSet}}$ is
unsatisfiable. Computing the FOL encodings of these judgments involves
the following intermediary steps: \begin{inparaenum} \item Encoding a
message history abstraction $\abstrace$ into an extended
consequent $\phidec$, i.e., $\atEncode{\abstrace}{\SpecSet} =
\phidec$.  \item Encoding a consequent $\phidec$
into a FOL formula $\psi$, i.e.,  $\toFOL{\phidec} = \psi$ \item For every specification $s\in\SpecSet$, $s$, for an
(existentially quantified) abstract message constant, $\absmsg$,
  resulting in a constraint on the message histories that end in
  $\absmsg$, i.e., $\instEncodeS{\absmsg}{s} \defeq \phidec$.
\item Applying the effect of a future message, $\absmsg$ to an already instantiated extended consequent, $\phidec_1$: 
$\updEncode{\phidec_1}{\absmsg} = \phidec_2$ \end{inparaenum}
For example state $R_2$:\rtwopre \ronepre \abstracebase from Section \ref{sec:overview} where \codej{unsubscribe} and \codej{call} must happen in the future. 
First, \codej{call} is instantiated to $[ \niDir{\enkwCi~s.\codej{unsubscribe()}}{\enkwCi~s := \codej{_.subscribe(}\absof{f}\codej{)}} ]$ and then the update for \codej{unsubscribe} is applied
$[ \niDir{\enkwCi~s.\codej{unsubscribe()}}{\enkwCi~s := \codej{_.subscribe(}\absof{f}\codej{)}} ] \wedge \codej{s} \neq \absof{s}$, finally, it is encoded to first order logic.


The first step, $\atEncode{\abstrace}{\SpecSet}$, encodes the
abstract trace into an intermediate representation, $\phidec$.  This
intermediate representation is an extension of the consequent from the
earlier section.  Existentials are added for the instantiation
operation operations that are introduced by instantiation.

\begin{small}
\[
\begin{array}{lrcll}
	\boxed{\atEncode{\abstrace}{\SpecSet} \defeq \directive}\\
	\atEncode{\abstracecons{\abstrace}{\absmsg}}{\SpecSet} & \defeq & \updEncode{\atEncode{\abstrace}{\SpecSet}}{\absmsg} \wedge \wedgeover{s \in \SpecSet} \instEncodeS{\absmsg}{s}\\ % \instEncode{\absmsg}{\SpecSet}\\
	\atEncode{\abstracebase}{\SpecSet} & \defeq & \text{true}\\
\end{array}
\]
 
\[
\begin{array}{lrcll}
%	\boxed{\instEncodeS{\absmsg}{s} \defeq \phidec}\\
	\instEncodeS{\absmsg_1}{\forall\ \lvars{x_1}.\ (\specOnly{\absmsg_2}{\exists\ \lvars{x_2}.\phi})}~\text{if}~
		\ideq{\absmsg_1}{\absmsg_2} & \defeq & \directive[\absmsg_2/\absmsg_1][\lvars{x_2}/\text{fresh}]\\
	\instEncodeS{\absmsg_1}{\forall\ \lvars{x_1}.\ (\specOnly{\absmsg_2}{\exists\ \lvars{x_2}.\phi})}~\text{if}~
		\idneq{\absmsg_1}{\absmsg_2} & \defeq & \enkwTrue\\
\end{array}
\]
\end{small}

In \instEncodeS{\absmsg}{s}, a single message and specification are
being instantiated. This eliminates the initial $\forall$ from the
\newls semantics in figure \ref{fig:cftl}.  This simplification can be
done because  $\exists y. \forall x. x=y \Rightarrow \text{p}(x)$ is
logically equivalent to $\exists y.  \text{p}(y)$.  We assume that the
arity of the target method must match if the framework name, $n$, and
direction, $g$, match.

The operator $[\absmsg_2/\absmsg_1]$ is used to indicate the operation
where each abstract value in the abstract message $\absmsg_2$ is
swapped for the corresponding value in $\absmsg_1$.  It is assumed
that no name collisions are possible, and the framework name and
message direction match.

To indicate the set of free variables in a consequent or abstract
message, we use $\mathtt{fv}(\absmsg)$.  In the case of
$\absof{v}`:=\enkwCi~n~\bar{\absof{v}}$, $\mathtt{fv}$ returns a set
of $\absof{v}'$ union with the elements in vector $\bar{\absof{v}}$.
An existential followed by a set is used to indicate an exists over
each variable in the set.



\begin{small}
\[
\begin{array}{lrcll}
	\boxed{\updEncode{\directive_1}{\absmsg} \defeq \directive_2} \\
	\updEncode{\iDir{\absmsg_1}}{\absmsg_2} & \defeq & (\absmsg_1 \neq \absmsg_2 \wedge \iDir{\absmsg_1}) \vee \absmsg_1 = \absmsg_2\\
	\updEncode{\niDir{\absmsg_1}{\absmsg_2}}{\absmsg_3} & \defeq & (\absmsg_1 = \absmsg_3 \vee (\absmsg_1 \neq \absmsg_3 \wedge \niDir{\absmsg_1}{\absmsg_2}))\\
	& & \wedge \absmsg_2 \neq \absmsg_3\\
	\updEncode{\notiDir{\absmsg_1}}{\absmsg_2} & \defeq & \notiDir{\absmsg_1} \wedge \absmsg_1 \neq \absmsg_2\\
	\updEncode{\directive_1 \wedge \directive_2}{\absmsg} & = & \updEncode{\directive_1}{\absmsg} \wedge \updEncode{\directive_2}{\absmsg}\\
	\updEncode{\directive_1 \vee \directive_2}{\absmsg} & \defeq & \updEncode{\directive_1}{\absmsg} \vee \updEncode{\directive_2}{\absmsg}\\
	\updEncode{\absmsg_1 = \absmsg_2}{\absmsg_3} & \defeq & \absmsg_1 = \absmsg_2 \\
	\updEncode{\forall x.~\phineg}{\absmsg} & \defeq & \forall x.~ \updEncode{ \phineg}{\absmsg}\\
	\updEncode{\exists x.~\directive}{\absmsg} & \defeq & \exists x.~ \updEncode{ \directive}{\absmsg}\\
\end{array}
\]
\end{small}




\fi

==> figures/appOnlyDiag.tex <==
\newcommand{\onedotstwo}{1 ~$...$~ 2}
\newcommand{\sixdots}{6 ~$...$~}
\newcommand{\aotrans}[1]{$#1$}
\newcommand{\vnodesep}{0.35cm}
\tikzset{location node/.style={draw=black, rounded corners, inner sep=0.2em, outer sep=0}}
\tikzset{msg node/.style={draw=none, inner sep=0, outer sep=-0.1em}}
\newcommand{\creTrans}{
\begin{tikzpicture}[]
\node (onc)[msg node] {\aotrans{\enkwCb~\codej{this.onCreate()}}};
\node (lone)[location node, below of=onc, node distance=\vnodesep]{\textit{1}};
\node (loneltwo)[below of=lone, node distance=\vnodesep]{\aotrans{\codej{this.act=$...$}}};
\node (ltwo)[location node, below of=loneltwo, node distance=\vnodesep]{\textit{2}};
\node (cre)[below of=ltwo, node distance=\vnodesep] {\aotrans{\codej{task=}\enkwCi~\codej{create($...$)}}};
\node (lthree)[location node, below of=cre, node distance=\vnodesep]{\textit{3}};
\node (sub)[below of=lthree, node distance=\vnodesep] {\aotrans{\codej{this.sub=}\enkwCi~\codej{tsk.subscribe(this)}}};
\node (lfour)[location node, below of=sub, node distance=\vnodesep]{\textit{4}};
\node (oncex)[below of=lfour, node distance=0.5cm]{\aotrans{\enkwCb\enkwRet~}};%~\codej{this.onCreate()}}};
% \draw[->] (onc) -- (lone);
% \draw[-] (lone) -- (loneltwo);
% \draw[->] (loneltwo) -- (ltwo);
% \draw[-] (ltwo) -- (cre);
% \draw[->] (cre) -- (crefwk);
% \draw[-] (crefwk) -- (creret);
% \draw[->] (creret) -- (lthree);
% \draw[-] (subfwk) -- (subret);
% \draw[-] (lthree) -- (sub);
% \draw[->] (subret) -- (lfour);
% \draw[->] (sub) -- (subfwk);
% \draw[-] (lfour) -- (oncex);
\end{tikzpicture}
}
\newcommand{\destTrans}{
\begin{tikzpicture}[every node/.style={rectangle, draw=none, rounded corners, every edge/.style={pos=0.4,draw=none}}]
\node (ond)[] {\aotrans{\enkwCb~\codej{this.onDestroy()}}};
\node (lsix)[location node, right of=ond, node distance=1.45cm]{\textit{6}};
\node (actnull)[right of=lsix, node distance=1cm]{\aotrans{\codej{this.act=null}}};
\node (lseven)[location node, right of=actnull, node distance=1.1cm]{\textit{7}};
\node (unsub)[right of=lseven, node distance=1.75cm] {\aotrans{\enkwCi~\codej{this.sub.unsubscribe()}}};
\node (unsubfwk)[location node, right of=unsub, node distance=1.95cm]{\ldots};
\node (unsubret)[right of=unsubfwk, node distance=0.6cm]{\enkwCi\enkwRet};
\node (leight)[location node, right of=unsubret, node distance=0.7cm]{\textit{8}};
\node (ondesx)[right of=leight, node distance=1.55cm]{\aotrans{\enkwCb\enkwRet~\codej{this.onDestroy()}}};
\draw[->] (ond) -- (lsix);
\draw[-] (lsix) -- (actnull);
\draw[->] (actnull) -- (lseven);
\draw[-] (lseven) -- (unsub);
\draw[->] (unsub) -- (unsubfwk);
\draw[-] (unsubfwk) -- (unsubret);
\draw[->] (unsubret) -- (leight);
\draw[-] (leight) -- (ondesx);
\end{tikzpicture}
}
\newcommand{\callTrans}{
\begin{tikzpicture}[every node/.style={rectangle, draw=none, rounded corners, every edge/.style={pos=0.4,draw=none}}]
\node (cal)[] {\aotrans{\enkwCb~\codej{this.call(m)}}};
\node (lfive)[location node, right of=cal, node distance=1.2cm]{\textit{5}};
\node (asrt)[right of=lfive, node distance=1.65cm]{\aotrans{\codej{assert(this.act != null)}}};
\node (dots)[right of=asrt, node distance=1.7cm]{~$...$~};
\node (calx)[right of=dots, node distance=1.45cm] {\aotrans{\enkwCb\enkwRet~\codej{this.call(m)}}};
\draw[->] (cal) -- (lfive);
\draw[-] (lfive) -- (asrt);
\draw[-] (asrt) -- (dots);
\draw[->] (dots) -- (calx);
\end{tikzpicture}
}
\begin{tikzpicture}[every node/.style={rectangle, draw=none, rounded corners, every edge/.style={pos=0.4,draw=none}}]
% \draw[help lines,step=5mm,gray!20] (0,0) grid (5,7);

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% [left nodes]
% \node (onc)[msg node] {\aotrans{\enkwCb~\codej{this.onCreate()}}};
\node (topleft)[node distance=\vnodesep/2] at (0,6.5) {};
\node (loneltwo)[location node, below of=topleft, node distance=\vnodesep]{\textit{\onedotstwo}};
\node (cre)[below of=loneltwo, node distance=\vnodesep] {\aotrans{\codej{task=}\enkwCi~\codej{create($...$)}}};
\node (lthree)[location node, below of=cre, node distance=\vnodesep]{\textit{3}};
\node (sub)[below of=lthree, node distance=\vnodesep] {\aotrans{\codej{this.sub=}\enkwCi~\codej{tsk.subscribe(this)}}};
\node (lfour)[location node, below of=sub, node distance=\vnodesep]{\textit{4}};
\node (bottomleft)[below of=lfour, node distance=\vnodesep/2]{};

% \node (oncex)[below of=lfour, node distance=0.5cm]{\aotrans{\aotrans{\enkwCb\enkwRet~\codej{this.onCreate()}}}};%~\codej{this.onCreate()}}};

\node (fwk) [location node, right=3 of cre.north east, node distance=4.2cm, text width=1.8cm, minimum height=2.5cm, minimum width = 2.0cm, anchor=north, draw]  {
    \begin{tabular}{l}
        \enkwFwk:\\
        $\{\refstate{1}:...\} \vee$ \\
        $\{\refstate{2}:...\} \vee$ \\
        $\{\refstate{3}:...\} \vee$ \\
        $\{\refstate{4}:...\} $\\
        \end{tabular}        
    };

% [Arrows of LEFT nodes]
% \draw[->, rounded corners] (fwk.north) - ++ (3,0) -- (3,-3) -- (loneltwo.north);
% \draw[->, rounded corners] (fwk.north) |- (-0.5, -0.5) 
%     node[yshift=0.2cm, xshift=-1cm] {\aotrans{\enkwCb~\codej{this.onCreate()}}} (loneltwo.north);
\draw[arrows = {-Stealth[harpoon]}, rounded corners] (fwk.120) |- node[yshift=0.15cm, xshift=-1.55cm] {\aotrans{\enkwCb~\codej{this.onCreate()}}} (loneltwo);
\draw[arrows = {Stealth[harpoon]-Stealth[harpoon]}] (cre) -- node[above=0.1mm] {ci} (fwk.134); % ci/ciret (left)
\draw[arrows = {Stealth[harpoon]-Stealth[harpoon]}] (sub) -- node[above=0.1mm] {ci} (fwk.161);% ci/ciret (left)
\draw[arrows = {-Stealth[harpoon]}, rounded corners] (lfour) -- node[anchor=north, xshift=0.19cm] {\aotrans{\enkwCb\enkwRet~\codej{this.onCreate()}}} (fwk.181); 

% [Boxes]
\node[draw,dotted, xshift=-0.15cm,  fit=(topleft.south) (loneltwo) (cre) (lthree) (sub) (lfour) (bottomleft) (fwk.210)] {};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% [Right nodes]
\node (topright)[node distance=\vnodesep/2] at (9.9,6.5) {};
% \node (rfive)[location node, node distance=\vnodesep] at (10.5,6) {\textit{5}};
\node (rfive)[location node, node distance=\vnodesep, below of=topright]{\textit{5}};
\node (cre)[below of=rfive, node distance=\vnodesep] {\aotrans{\codej{assert(this.act != null)}}};
% \node (rsixactset)[below of=cre, node distance=\vnodesep] {\aotrans{\codej{$...$}}};
\node (rsixactset)[location node, below of=cre, node distance=\vnodesep] {\textit{\sixdots}};

\node (rseven)[location node, right=3 of fwk.-4, node distance=125.0]{\textit{7}};
\node (actnull)[below of=rseven, node distance=\vnodesep]{\aotrans{\codej{this.act=null}}};

\node (reight)[location node, below of=actnull, node distance=\vnodesep]{\textit{8}};
\node (unsub)[below of=reight, node distance=\vnodesep] {\aotrans{\codej{this.sub.unsubscribe()}}};
\node (rnine)[location node, below of=unsub, node distance=\vnodesep]{\textit{9}};
\node (bottomright)[below of=rnine, node distance=\vnodesep/2]{};


% [Arrows of right nodes]
\draw[arrows = {-Stealth[harpoon]}, rounded corners] (fwk.63) |- node[yshift=0.15cm, xshift=3.8cm] {\aotrans{\enkwCb~\codej{this.call(m)}}} (rfive); 
\draw[arrows = {-Stealth[harpoon]}, rounded corners] (rsixactset) -- node[anchor=north, yshift=0.05cm, xshift=1.1cm] {\aotrans{\enkwCb\enkwRet~\codej{this.call(m)}}} (fwk.34.5);
\draw[arrows = {-Stealth[harpoon]}, rounded corners] (fwk.-4) -- node[anchor=west, yshift=0.15cm, xshift=-1.2cm] {\aotrans{\enkwCb~\codej{this.onDestroy()}}} (rseven); 
\draw[arrows = {Stealth[harpoon]-Stealth[harpoon]}] (unsub.180) -- node[above=0.1mm] {ci} (fwk.312.5); % ci (right)
\draw[arrows = {-Stealth[harpoon]}, rounded corners] (rnine) -| node[anchor=west, yshift=-0.15cm,  xshift=1.1cm] {\aotrans{\enkwCb\enkwRet~\codej{this.onDestroy()}}} (fwk.south); 

% [Boxes]
\node[draw,dotted, xshift=0.15cm,  fit=(topright.south) (rfive) (cre) (rsixactset) (fwk.22)] {};
\node[draw,dotted, xshift=0.15cm,  fit=(rseven) (actnull) (reight) (unsub) (rnine) (bottomright) (fwk.10)] {};

% \draw[->, rounded corners] (fwk.north)  (0,0) -- (0pt,25pt) -- (40pt,25pt) node[yshift=0.2cm, xshift=-1cm] {\aotrans{\enkwCb~\codej{this.onCreate()}}} (loneltwo.north);
% \draw (0,0) -- (2ex,0pt) -- +(up:1ex);
%\node (cretrans)[left of=fwk, node distance=3cm, outer sep=0, inner sep=0]{\creTrans};
% \node (calltrans)[below of=fwk, node distance=0.5cm, outer sep=0, inner sep=0]{\callTrans};
% \node (desttrans)[below of=fwk, node distance=1cm, outer sep=0, inner sep=0]{\destTrans}; 
% 
% \draw[-,rounded corners] (fwk.west) - ++ (-3.45,0) |- (cretrans.west);
% \draw[->,rounded corners] (cretrans.east) - ++ (0.08,0) -- ++ (0.08,-0.5) -- (fwk.east);
% \draw[-,rounded corners] (fwk.west) - ++ (-3,0) |- (desttrans.west);
% \draw[->,rounded corners] (desttrans.east) - ++ (0.40,0) -- ++ (0.40,1) -- (fwk.east);
% \draw[-,rounded corners] (fwk.west) - ++ (-1,0) |- (calltrans.west);
% \draw[->,rounded corners] (calltrans.east) - ++ (0.15,0) -- ++ (0.15,0.5) -- (fwk.east);


\end{tikzpicture}


==> figures/appOnlyDiag_old.tex <==

\newcommand{\aotrans}[1]{$#1$}
\newcommand{\vnodesep}{0.35cm}
\tikzset{location node/.style={draw=black, rounded corners, inner sep=0.2em, outer sep=0}}
\tikzset{msg node/.style={draw=none, inner sep=0, outer sep=-0.1em}}
\newcommand{\creTrans}{
\begin{tikzpicture}[]
\node (onc)[msg node] {\aotrans{\enkwCb~\codej{this.onCreate()}}};
\node (lone)[location node, below of=onc, node distance=\vnodesep]{\textit{1}};
\node (actset)[below of=lone, node distance=\vnodesep]{\aotrans{\codej{this.act=$...$}}};
\node (ltwo)[location node, below of=actset, node distance=\vnodesep]{\textit{2}};
\node (cre)[below of=ltwo, node distance=\vnodesep] {\aotrans{\codej{task=}\enkwCi~\codej{create($...$)}}};
\node (lthree)[location node, below of=cre, node distance=\vnodesep]{\textit{3}};
\node (sub)[below of=lthree, node distance=\vnodesep] {\aotrans{\codej{this.sub=}\enkwCi~\codej{tsk.subscribe(this)}}};
\node (lfour)[location node, below of=sub, node distance=\vnodesep]{\textit{4}};
\node (oncex)[below of=lfour, node distance=0.5cm]{\aotrans{\enkwCb\enkwRet~}};%~\codej{this.onCreate()}}};
% \draw[->] (onc) -- (lone);
% \draw[-] (lone) -- (actset);
% \draw[->] (actset) -- (ltwo);
% \draw[-] (ltwo) -- (cre);
% \draw[->] (cre) -- (crefwk);
% \draw[-] (crefwk) -- (creret);
% \draw[->] (creret) -- (lthree);
% \draw[-] (subfwk) -- (subret);
% \draw[-] (lthree) -- (sub);
% \draw[->] (subret) -- (lfour);
% \draw[->] (sub) -- (subfwk);
% \draw[-] (lfour) -- (oncex);
\end{tikzpicture}
}
\newcommand{\destTrans}{
\begin{tikzpicture}[every node/.style={rectangle, draw=none, rounded corners, every edge/.style={pos=0.4,draw=none}}]
\node (ond)[] {\aotrans{\enkwCb~\codej{this.onDestroy()}}};
\node (lsix)[location node, right of=ond, node distance=1.45cm]{\textit{6}};
\node (actnull)[right of=lsix, node distance=1cm]{\aotrans{\codej{this.act=null}}};
\node (lseven)[location node, right of=actnull, node distance=1.1cm]{\textit{7}};
\node (unsub)[right of=lseven, node distance=1.75cm] {\aotrans{\enkwCi~\codej{this.sub.unsubscribe()}}};
\node (unsubfwk)[location node, right of=unsub, node distance=1.95cm]{\ldots};
\node (unsubret)[right of=unsubfwk, node distance=0.6cm]{\enkwCi\enkwRet};
\node (leight)[location node, right of=unsubret, node distance=0.7cm]{\textit{8}};
\node (ondesx)[right of=leight, node distance=1.55cm]{\aotrans{\enkwCb\enkwRet~\codej{this.onDestroy()}}};
\draw[->] (ond) -- (lsix);
\draw[-] (lsix) -- (actnull);
\draw[->] (actnull) -- (lseven);
\draw[-] (lseven) -- (unsub);
\draw[->] (unsub) -- (unsubfwk);
\draw[-] (unsubfwk) -- (unsubret);
\draw[->] (unsubret) -- (leight);
\draw[-] (leight) -- (ondesx);
\end{tikzpicture}
}
\newcommand{\callTrans}{
\begin{tikzpicture}[every node/.style={rectangle, draw=none, rounded corners, every edge/.style={pos=0.4,draw=none}}]
\node (cal)[] {\aotrans{\enkwCb~\codej{this.call(m)}}};
\node (lfive)[location node, right of=cal, node distance=1.2cm]{\textit{5}};
\node (asrt)[right of=lfive, node distance=1.65cm]{\aotrans{\codej{assert(this.act != null)}}};
\node (dots)[right of=asrt, node distance=1.7cm]{~$...$~};
\node (calx)[right of=dots, node distance=1.45cm] {\aotrans{\enkwCb\enkwRet~\codej{this.call(m)}}};
\draw[->] (cal) -- (lfive);
\draw[-] (lfive) -- (asrt);
\draw[-] (asrt) -- (dots);
\draw[->] (dots) -- (calx);
\end{tikzpicture}
}
\begin{tikzpicture}[every node/.style={rectangle, draw=none, rounded corners, every edge/.style={pos=0.4,draw=none}}]
\draw[help lines,step=5mm,gray!20] (0,0) grid (5,7);
% \node (onc)[msg node] {\aotrans{\enkwCb~\codej{this.onCreate()}}};
\node (actset)[node distance=\vnodesep] at (0,6) {\aotrans{\codej{$...$}}};
\node (lone)[location node, left of=actset, node distance=\vnodesep]{\textit{1}};
\node (ltwo)[location node, right of=actset, node distance=\vnodesep]{\textit{2}};
\node (cre)[below of=actset, node distance=\vnodesep] {\aotrans{\codej{task=}\enkwCi~\codej{create($...$)}}};
\node (lthree)[location node, below of=cre, node distance=\vnodesep]{\textit{3}};
\node (sub)[below of=lthree, node distance=\vnodesep] {\aotrans{\codej{this.sub=}\enkwCi~\codej{tsk.subscribe(this)}}};
\node (lfour)[location node, below of=sub, node distance=\vnodesep]{\textit{4}};
\node (oncex)[below of=lfour, node distance=0.5cm]{\aotrans{\enkwCb\enkwRet~}};%~\codej{this.onCreate()}}};

\node (fwk)[location node, right of=lthree, node distance=3cm, text width=2.25cm] {$\enkwFwk: \{\refstate{1}:...\} \vee \{\refstate{2}:...\} \vee \{\refstate{3}:...\} \vee \{\refstate{4}:...\}$};

\draw[->, rounded corners] (fwk.north) - ++ (3,0) -- (3,-3) -- (actset.north);
%\node (cretrans)[left of=fwk, node distance=3cm, outer sep=0, inner sep=0]{\creTrans};
% \node (calltrans)[below of=fwk, node distance=0.5cm, outer sep=0, inner sep=0]{\callTrans};
% \node (desttrans)[below of=fwk, node distance=1cm, outer sep=0, inner sep=0]{\destTrans}; 
% 
% \draw[-,rounded corners] (fwk.west) - ++ (-3.45,0) |- (cretrans.west);
% \draw[->,rounded corners] (cretrans.east) - ++ (0.08,0) -- ++ (0.08,-0.5) -- (fwk.east);
% \draw[-,rounded corners] (fwk.west) - ++ (-3,0) |- (desttrans.west);
% \draw[->,rounded corners] (desttrans.east) - ++ (0.40,0) -- ++ (0.40,1) -- (fwk.east);
% \draw[-,rounded corners] (fwk.west) - ++ (-1,0) |- (calltrans.west);
% \draw[->,rounded corners] (calltrans.east) - ++ (0.15,0) -- ++ (0.15,0.5) -- (fwk.east);


\end{tikzpicture}


==> figures/fwkNodeAP.tex <==
\newcommand{\loopsp}{35}
\newcommand{\createDeg}{90+45+\loopsp/2}
\newcommand{\callDeg}{90-45 + \loopsp/2}
\newcommand{\subDeg}{270-45+\loopsp/2}
\newcommand{\unsubDeg}{270+45+\loopsp/2}
\newcommand{\lset}{7}

% Macro that expands to computation of angles for each edge
\newcommand{\edgeset}[2]{edge[#2,out=#1,in=#1-\loopsp, looseness=\lset]}
\begin{tikzpicture}[node distance=3cm]
	\node[state, accepting, initial] (q2) {\codej{Single}};
	\path[->] (q2) \edgeset{\callDeg}{loop right} node{\enkwCb \codej{\_.call()}} (q2);
	\path[->] (q2) \edgeset{\createDeg}{loop above} node{\enkwCi \codej{ \_ = create(\_)}} (q2);
	\path[->] (q2) \edgeset{\subDeg}{loop below} node{\enkwCi \codej{\_.subscribe(\_)}} (q2);
	\path[->] (q2) \edgeset{\unsubDeg}{loop right} node{\enkwCi \codej{\_.unsubscribe()}} (q2);
\end{tikzpicture}


==> figures/proofTreeNoSpec.tex <==
\newcommand{\lambdaShort}{
\begin{tabular}{l}
\enkwCb~\codej{l.lambda(s)}\\
\codej{assert(l.outer.mediaName != null)}
\end{tabular}
}
\newcommand{\initShort}{
	\begin{tabular}{l}
	\enkwCb~\codej{f.<init>()}\\
	\codej{f.mediaName := }\enkwNull\\
	\codej{f.sub := } \enkwNull\\
	\codej{f.act := } \enkwNull\\
	%\enkwCi~\codej{f.sub.unsubscribe()}\\
	%\codej{f.act =} \enkwNull\\
	\end{tabular}
}
\newcommand{\oncFull}{
	\begin{tabular}{l}
	\enkwCb~\codej{f.onCreate()}\\
	\codej{tmp1 := new lambda(f)}
	\codej{tmp2 := }\enkwCi~\codej{create(tmp1)}\\
	\codej{f.sub := }\enkwCi~\codej{tmp2.subscribe(f)}\\
	\end{tabular}
}
\newcommand{\subs}{
\begin{tabular}{c}
$\entail{\refstate_4}{\refstate_3}$\\%(case \codej{onCreate})
\end{tabular}
}

\begin{tikzpicture}[node distance=0.80cm, every node/.style={rectangle, draw=black, rounded corners, every edge/.style={pos=0.4,draw=none}}]
\node (lambda)[text width=4.75cm] {\lambdaShort};
\node (R1)[above of=lambda, draw=none, node distance = 1.2cm] {
\begin{minipage}{5.8cm}
$\refstate_1:\absof{l}.\codej{outer} \mapsto \absof{f} \ast \absof{f}.\codej{mediaName} \mapsto \enkwNull \wedge \abstracebase $
\end{minipage}
};
\node (init)[above of=R1, text width=3cm, node distance=1.9cm]{\initShort};
\node (R2)[above of=init, draw=none, node distance=1.7cm] {
\begin{minipage}{3cm}
$\refstate_2:\absof{l}.\codej{outer} \mapsto \absof{f} \wedge \abstracebase $
\end{minipage}
};
\node (other)[right of=init, node distance=3.5cm]{...};

\path[-)] (R1) edge (lambda);
\path[-)] (R2) edge (init);
\draw (init) edge[-] node[draw=none,left]{
\begin{minipage}{3.5cm}
(case: \codej{<init>} and \codej{f} $\mapsto \absof{f}$)
\end{minipage}
} (R1);
\draw (other) edge[-] node[draw=none,right]{
\begin{minipage}{1cm}
(case: other)
\end{minipage}
} (R1.east);
\end{tikzpicture}


==> generated/msgCountTable.tex <==
\newcommand{\classtilt}{90}
\newcommand{\codejp}[1]{
\begin{minipage}{4cm}
\codej{#1}
\end{minipage}
}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l r r r r r r r r r }
& \multicolumn{9}{l}{Framework Object}\\
Spec&\rotatebox{\classtilt}{\codejp{Action1}}&\rotatebox{\classtilt}{\codejp{Activity}}&\rotatebox{\classtilt}{\codejp{AsyncTask}}&\rotatebox{\classtilt}{\codejp{Dialog}}&\rotatebox{\classtilt}{\codejp{Fragment}}&\rotatebox{\classtilt}{\codejp{OnClickListener}}&\rotatebox{\classtilt}{\codejp{Single}}&\rotatebox{\classtilt}{\codejp{Subscription}}&\rotatebox{\classtilt}{\codejp{View}}\\
\toprule
\ref{spec:call}&1&&&&&&1&1&\\
\ref{spec:createOnce}&&1&&&&&&&\\
\ref{spec:clickFinish}&&4&&&&1&&&1\\
\ref{spec:clickDisable}&&&&&&1&&&2\\
\ref{spec:findView}&&1&&&&&&&\\
\ref{spec:getActivityNull}&&&&&3&&&&\\
\ref{spec:execute}&&&1&&&&&&\\
\ref{spec:show}&&&&1&&&&&\\
\ref{spec:dismiss}&&2&&2&&&&&\\
\ref{spec:onActivityCreated}&&&&&2&&&&\\
\midrule
used&1&5&1&2&3&1&1&1&2\\
possible&1&703&42&191&203&1&139&35&1099\\
\bottomrule
\end{tabular*}


==> macros.tex <==
% -*-latex-*-
\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Tikz Stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzstyle{lastate}=[state,accepting,scale=0.3]
\tikzstyle{lainitial}=[initial,initial text={}, initial where=above]
\tikzstyle{lalabel}=[scale=1]

\tikzstyle{pfsainitial}=[initial,initial text={$I(x_1):1$}, initial where=above]
\tikzstyle{pfsainitialabove}=[initial,initial text={$I_\mathcal{A}:1$}, initial where=above]
\tikzstyle{pfsainitialleft}=[initial,initial text={$I_\mathcal{A}:1$}, initial where=left]
\tikzstyle{pfsainitialright}=[initial,initial text={$I_\mathcal{A}:1$}, initial where=right]
\tikzstyle{pfsafinal}=[hmmstate,accepting]
\tikzstyle{observation}=[shape=rectangle,draw=orange!50,fill=orange!20]
\tikzstyle{lightedge}=[<-,dotted]
\tikzstyle{mainstate}=[state,thick]
\tikzstyle{mainedge}=[<-,thick]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Listing Stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\toolname}{\textsc{Historia}\xspace} %%%TODO: come up with a better name
%\newcommand{\toolinfer}{\textit{Infer}\xspace}
\newcommand{\toolinfer}{Infer\xspace}
\newcommand{\toolflowdroid}{Flowdroid\xspace}
\theoremstyle{definition}
\newtheorem{specDef}{History Implication}
\newtheorem{assumption}{Assumption}
\newtheorem{property}{Property}
%\newcommand{\specbox}[1]{\parbox[t]{0.75\textwidth}{%
%    \setstretch{1.33}\raggedright$\displaystyle \hspace{-0.3cm}#1$}}
\newcommand{\specbox}[1]{\par\noindent\parbox{\linewidth}{\centering\vspace{\abovedisplayskip}\parbox{0.9\linewidth}{%
\raggedright$\displaystyle #1$}}}
%%% Syntax
\lstdefinelanguage{Enable}{
  morekeywords={in,if,then,else,new,bind,invoke,skip,assume,enable,disable,allow,disallow,true,false,me,app,fwk,event,callback,callin,force,assert,null,reach, unreach},
  literate={pskip}{{$\bullet$}}1
}

\newcommand{\cbstyle}{\colordullx{0}}
\newcommand{\cistyle}{\colordullx{4}}
\newcommand{\fwktystyle}{\colordullx{1}\relsize{-1}}
%\newcommand{\evtstyle}{\normalfont\ttfamily\scshape}
\lstdefinelanguage{exthighlighting}[]{highlighting}{%
  moredelim=**[is][\cbstyle]{|cb:}{|},
  moredelim=**[is][\cistyle]{|ci:}{|},
  moredelim=**[is][\fwktystyle]{|fwkty:}{|},
  moredelim=*[is][\evtstyle]{|evt:}{|},
  morekeywords={assert,var},
}

\lstset{
  breaklines=true,
  emphstyle=\cbstyle,
  emph={onStop,lambda,onActivityCreated,onCreate,subs,run,getActionBar,onStart,onResume,onPause,onDestroy,oD,oAC,onClick,onPrepared,onError,doInBackground,onPostExecute,init,call},
  emphstyle={[2]\cistyle},
  emph={[2]setOnClickListener,dispose,subscribeOn,observeOn,show,dismiss,setOnClickList,return_onResume,setOnPreparedListener,reset,start,setEnabled,enable,disable,setDataSource,prepareAsync,execute,cancel, unsubscribe,<init>,getResources,getWidth,finish,setResult,findViewById,setEnable,getActivity,getAct, create, subscribe, with, load, showFragment},
  emphstyle={[3]\fwktystyle},
  emph={[3]Activity,Bundle,Button,AsyncTask,Handler,OnClickListener,View,Fragment,Maybe, Single,Glide,Subscription,Subscriber,Action1,Dialog,Runnable}
}

%\newcommand{\codex}[2]{\ensuremath{\text{\lstinline[#1]~#2~}}}
\newcommand{\codej}[1]{\codex{language=Java,alsolanguage=exthighlighting,breaklines=true}{#1}}
\newcommand{\coden}[1]{\codex{language=Enable,alsolanguage=exthighlighting}{#1}}
\newcommand{\enmkkw}[2]{\savebox{#1}{\coden{#2}}}

\newcommand{\codejmk}[3][\relax]{\sbox#2{#1\codej{#3}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Concrete Model
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\subst}[2]{\ensuremath{[#1/#2]}}

% Maps
\newcommand{\map}[1]{\ensuremath{[#1]}}
\newcommand{\maplet}[2]{\ensuremath{#1 \mathbin{\mapsto} #2}}
%\newcommand{\empmap}{\ensuremath{\map{\,}}}
\newcommand{\empmap}{\ensuremath{\circ}}
\newcommand{\extmap}[2]{\ensuremath{[\maplet{#1}{#2}]}}
\newcommand{\maplookup}[2]{\ensuremath{#1(#2)}}
%\newcommand{\mapupdate}[3]{\ensuremath{#1(#2 \gets #3)}}
\newcommand{\MapST}[2]{\ensuremath{\left[\,#1 \SuchThat{#1}{#2} #2\,\right]}}

%%% Meta Variables
\newcommand{\app}{\ensuremath{\mathit{app}}}
\newcommand{\cb}{\ensuremath{\mathit{cb}}}
\newcommand{\term}{\ensuremath{t}}
\newcommand{\expr}{\ensuremath{e}}
\newcommand{\ExprSet}{\SetName{Expr}}
\newcommand{\var}{\ensuremath{x}}
\newcommand{\VarSet}{\SetName{Var}}
\newcommand{\fld}{\ensuremath{f}}
\newcommand{\FldSet}{\SetName{Field}}
\newcommand{\cont}{\ensuremath{c}}
\newcommand{\ContSet}{\SetName{Cont}}
\newcommand{\val}{\ensuremath{v}}
\newcommand{\ValSet}{\SetName{Val}}
\newcommand{\addr}{\ensuremath{a}}
\newcommand{\AddrSet}{\SetName{Addr}}
\newcommand{\stack}{\ensuremath{\kappa}}
\newcommand{\ThunkSet}{\SetName{Thunk}}
\newcommand{\handle}{\ensuremath{h}}
\newcommand{\HandleSet}{\SetName{Handle}}
\newcommand{\msg}{\ensuremath{m}}
\newcommand{\MsgSet}{\SetName{Msg}}
\newcommand{\pkg}{\ensuremath{g}}
%\newcommand{\trans}{\ensuremath{\tau}}
\newcommand{\transset}{\ensuremath{T}}
\newcommand{\TransSet}{\SetName{Trans}}
\newcommand{\absTransSet}{\absofset{\TransSet}}
\newcommand{\observe}{\ensuremath{o}}
\newcommand{\ObserveSet}{\SetName{Observable}}
\newcommand{\obsty}{\MVar{oknd}}
\newcommand{\statepath}{\ensuremath{\pi}}
\newcommand{\lpath}{pth}
\newcommand{\statepathset}{\ensuremath{\Pi}}
\newcommand{\PathSet}{\SetName{Path}}
\newcommand{\trace}{\ensuremath{\varpi}}
\newcommand{\abstrace}{\ensuremath{\absof{\omega}}}
%\newcommand{\abstracebase}{\ensuremath{\bigcirc}}
\newcommand{\abstracebase}{\fmtlogicconst{okhist}}
\newcommand{\abstracecons}[2]{\ensuremath{#2 \twoheadrightarrow #1}} % right-implication
%\newcommand{\traceset}{\ensuremath{\varPi}}
\newcommand{\abstraceset}{\ensuremath{\varPi}}
\newcommand{\TraceSet}{\SetName{Trace}}
\newcommand{\absTransSeqSet}{\ensuremath{\seqof{\absofset{\TransSet}}}}
\newcommand{\obstrace}{\ensuremath{\theta}}
\newcommand{\obstraceset}{\ensuremath{\Theta}}
\newcommand{\ObsTraceSet}{\SetName{Observ}}
\newcommand{\weight}{\ensuremath{w}}
\newcommand{\tytag}{\ensuremath{T}}
\newcommand{\TytagSet}{\SetName{Tag}}

%% distilled syntax
\newcommand{\fmtmvar}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\fmttxtsub}[1]{\ensuremath{\textrm{#1}}}
\newcommand{\trans}{\fmtmvar{t}}
\newcommand{\btrans}{\fmtmvar{b}}
\newcommand{\msgid}{\fmtmvar{md}}
\newcommand{\msgcall}[2]{\ensuremath{#1(#2)}}
\newcommand{\msgcallret}[3]{\ensuremath{#1\,\msgcall{#2}{#3}}}
\newcommand{\msgcb}[2]{\ensuremath{\enkwCb\,\msgcall{#1}{#2}}}
\newcommand{\msgci}[3]{\ensuremath{\enkwCi\,\msgcallret{#1}{#2}{#3}}}
\newcommand{\msgcbret}[3]{\ensuremath{\enkwCb\enkwRet\,\msgcallret{#1}{#2}{#3}}}
% \newcommand{\msgcbret}[3]{\ensuremath{\enkwCb\enkwRet\,\msgcallret{}{#2}{#3}}} % remove call return for now, wasn't needed for examples
\newcommand{\cbretcmd}[1]{\ensuremath{\enkwCb\enkwRet\,#1}}
\newcommand{\fmtseq}[1]{\ensuremath{\overline{#1}}}
\newcommand{\valseq}{\fmtseq{\val}}
\newcommand{\varseq}{\fmtseq{\var}}
\newcommand{\loc}{\fmtmvar{loc}}
\newcommand{\apploc}{\fmtmvar{\ell}}
\newcommand{\prog}{\fmtmvar{p}}
\newcommand{\progemp}{\circ}
\newcommand{\progcons}[2]{\ensuremath{#1, #2}}
\newcommand{\histfolmodel}{\omega_{\mathtt{FOL}}}
\newcommand{\hist}{\omega}
\newcommand{\histemp}{\varepsilon}
\newcommand{\histcons}[2]{\ensuremath{#1; #2}}
\newcommand{\msgstack}{\kappa}
\newcommand{\msgstackframe}{\fmtmvar{k}}
\newcommand{\msgstackemp}{\circ}
\newcommand{\msgstackcons}[2]{\ensuremath{#1; #2}}
\newcommand{\appstore}{\rho}
\newcommand{\inittxtsub}{\text{\fmttxtsub{init}}}

\newcommand{\initappstore}{\appstore_\inittxtsub}
\newcommand{\appstate}{\varsigma}
\newcommand{\mem}{\mu}
\newcommand{\mkmem}[3]{#1 \cdot #3 \cdot #2}
\newcommand{\pstate}{\sigma}
\newcommand{\initpstate}{\pstate_\inittxtsub}
\newcommand{\mkappstate}[2]{#2\colon #1}
\newcommand{\mkpstate}[4]{#4\colon \mkmem{#1}{#2}{#3}}
\newcommand{\mkpstatemem}[2]{#2\colon #1}
\newcommand{\mklocstate}[2]{#2\colon #1}
\newcommand{\appval}{\fmtmvar{a}}
\newcommand{\fwkval}{\fmtmvar{f}}

\newcommand{\preop}{\operatorname{pre}}
\newcommand{\postop}{\operatorname{post}}
\newcommand{\preof}[1]{\preop(#1)}
\newcommand{\postof}[1]{\postop(#1)}

\newcommand{\SpecSet}{\ensuremath{S}}

\newcommand{\spec}{\ensuremath{s}}
\newcommand{\spectrue}{\ensuremath{\text{true}}}
\newcommand{\specOnly}[2]{#1 \ensuremath{\boxright} #2}
\newcommand{\iDir}[1]{\ensuremath{\mathbf{O}~#1}}
\newcommand{\notiDir}[1]{\ensuremath{\mathbf{HN}~#1}}
\newcommand{\niDir}[2]{\ensuremath{#1~\mathbf{NS}~#2}}

\newcommand{\env}{\ensuremath{\eta}}
\newcommand{\EnvSet}{\SetName{Env}}
\newcommand{\store}{\ensuremath{\rho}}
\newcommand{\StoreSet}{\SetName{Store}}
\newcommand{\eventmap}{\ensuremath{\mu}}
\newcommand{\EventmapSet}{\SetName{Enabled}}
\newcommand{\callinmap}{\ensuremath{\nu}}
\newcommand{\CallinmapSet}{\SetName{Allowed}}

\newcommand{\fmtevt}[1]{\ensuremath{\text{\evtstyle #1}}}
\newcommand{\evtcb}[2]{\enFrame{\fmtevt{#1}}{#2}}

\newcommand{\refstate}[1]{\ensuremath{\quies_{#1}}}
\newcommand{\refapploc}[1]{\ensuremath{\ensuremath{\mathtt{point}\text{-}#1}}}
\newcommand{\LabelSet}{\SetName{Label}}

\newsavebox{\@enkwErr}\enmkkw{\@enkwErr}{exn}
\newcommand{\enkwErr}{\usebox{\@enkwErr}}
\newsavebox{\@enkwNew}\enmkkw{\@enkwNew}{new}
\newcommand{\enkwNew}{\usebox{\@enkwNew}}
\newsavebox{\@enkwNull}\enmkkw{\@enkwNull}{null}
\newcommand{\enkwNull}{\usebox{\@enkwNull}}
\newsavebox{\@enkwInvoke}\enmkkw{\@enkwInvoke}{invoke}
\newcommand{\enkwInvoke}{\usebox{\@enkwInvoke}}
\newsavebox{\@enkwSkip}\enmkkw{\@enkwSkip}{skip}
\newcommand{\enkwSkip}{\usebox{\@enkwSkip}}
\newsavebox{\@enkwAssume}\enmkkw{\@enkwAssume}{assume}
\newcommand{\enkwAssume}{\usebox{\@enkwAssume}}
\newsavebox{\@enkwEnable}\enmkkw{\@enkwEnable}{enable}
\newcommand{\enkwEnable}{\usebox{\@enkwEnable}}
\newsavebox{\@enkwAssert}\enmkkw{\@enkwAssert}{assert}
\newcommand{\enkwAssert}{\usebox{\@enkwAssert}}
\newsavebox{\@enkwDisable}\enmkkw{\@enkwDisable}{disable}
\newcommand{\enkwDisable}{\usebox{\@enkwDisable}}
\newsavebox{\@enkwAllow}\enmkkw{\@enkwAllow}{allow}
\newcommand{\enkwAllow}{\usebox{\@enkwAllow}}
\newsavebox{\@enkwDisallow}\enmkkw{\@enkwDisallow}{disallow}
\newcommand{\enkwDisallow}{\usebox{\@enkwDisallow}}
\newsavebox{\@enkwForce}\enmkkw{\@enkwForce}{force}
\newcommand{\enkwForce}{\usebox{\@enkwForce}}
\newsavebox{\@enkwTrue}\enmkkw{\@enkwTrue}{true}
\newcommand{\enkwTrue}{\usebox{\@enkwTrue}}
\newsavebox{\@enkwFalse}\enmkkw{\@enkwFalse}{false}
\newcommand{\enkwFalse}{\usebox{\@enkwFalse}}
\newsavebox{\@enkwMe}\enmkkw{\@enkwMe}{me}
\newcommand{\enkwMe}{\usebox{\@enkwMe}}
\newsavebox{\@enkwApp}\enmkkw{\@enkwApp}{app}
\newcommand{\enkwApp}{\usebox{\@enkwApp}}
\newsavebox{\@enkwFwk}\enmkkw{\@enkwFwk}{fwk}
\newcommand{\enkwFwk}{\usebox{\@enkwFwk}}
\newsavebox{\@enkwEvent}\enmkkw{\@enkwEvent}{event}
\newcommand{\enkwEvent}{\usebox{\@enkwEvent}}
\newsavebox{\@enkwCallback}\enmkkw{\@enkwCallback}{callback}
\newcommand{\enkwCallback}{\usebox{\@enkwCallback}}
\newsavebox{\@enkwCallin}\enmkkw{\@enkwCallin}{callin}
\newcommand{\enkwCallin}{\usebox{\@enkwCallin}}
\newcommand{\enkwIndent}{\hspace{2em}}

\newcommand{\fmtstate}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\enkwDisallowed}{\fmtstate{disallowed}}
\newcommand{\enkwInitial}{\fmtstate{initial}}

\newcommand{\enLet}[3]{\ensuremath{\enkwLet\;#1\;\pcode{=}\;#2\;\enkwIn\;#3}}
\newcommand{\enGetf}[2]{\ensuremath{#1\pcode{.}#2}}
\newcommand{\enPutf}[3]{\ensuremath{#1\pcode{.}#2\;\pcode{=}\;#3}}
\newcommand{\enNew}{\enkwNew}
\newcommand{\enSkipK}{\ensuremath{\bullet}}
\newcommand{\enSkip}{\ensuremath{()}}
\newcommand{\enSeq}[2]{\ensuremath{#1\pcode{;}\,#2}}
\newcommand{\enIf}[3]{\ensuremath{\enkwIf\;#1\;\enkwThen\;#2\;\enkwElse\;#3}}
\newcommand{\enBind}[3][]{\ensuremath{\enkwBind_{#1}\;#2\;#3}}
\newcommand{\enInvoke}[2]{\ensuremath{\enkwInvoke\;#1\;#2}}
\newcommand{\enEnable}[1]{\ensuremath{\enkwEnable\;#1}}
\newcommand{\enDisable}[1]{\ensuremath{\enkwDisable\;#1}}
\newcommand{\enAllow}[1]{\ensuremath{\enkwAllow\;#1}}
\newcommand{\enDisallow}[1]{\ensuremath{\enkwDisallow\;#1}}
\newcommand{\enFun}[3][\pkg]{\ensuremath{#2\Rightarrow_{#1}#3}}
\newcommand{\enForce}[1]{\ensuremath{\enkwForce\;#1}}
\newcommand{\enTrue}{\enkwTrue}
\newcommand{\enFalse}{\enkwFalse}
\newcommand{\enMe}{\enkwMe}
\newcommand{\enApp}{\enkwApp}
\newcommand{\enAppSub}{\ensuremath{\mathbf{app}}}
\newcommand{\enFwk}{\enkwFwk}
\newcommand{\enFwkSub}{\ensuremath{\mathbf{fwk}}}
%\newcommand{\enEvent}[1]{\ensuremath{\enkwEvent\;#1}}
%\newcommand{\enCallback}[1]{\ensuremath{\enkwCallback\;#1}}
%\newcommand{\enCallin}[1]{\ensuremath{\enkwCallin\;#1}}
\newcommand{\enEvent}{\enkwEvent}
\newcommand{\enCallin}{\enkwCallin}
\newcommand{\enInitial}{\enkwInitial}
\newcommand{\enDisallowed}{\enkwDisallowed}
\newcommand{\enCallback}{\enkwCallback}
\newcommand{\enAddr}{\ensuremath{addr}}

%\newcommand{\enClosure}[2]{\ensuremath{#1[#2]}}
\newcommand{\enClosure}[2]{\ensuremath{#1}}
\newcommand{\enMsg}[2]{\ensuremath{(#1,#2)}}
\newcommand{\extMsg}[2]{\ensuremath{[\enMsg{#1}{#2}]}}
%\newcommand{\ext}[1]{\ensuremath{[#1]}}
\newcommand{\ext}[1]{\ensuremath{, #1}}
%\newcommand{\enMsg}[2]{\ensuremath{#1 #2}}
\newcommand{\enThunk}[2]{\ensuremath{#1[#2]}}
\newcommand{\frameop}{\mathord{\gg}}
\newcommand{\enFrame}[2]{\ensuremath{#1\frameop#2}}

\newcommand{\enLetK}[3]{\ensuremath{\enkwLet\;#1\;\pcode{=}\;#2\;\enkwIn\;#3}}

\newcommand{\@enState}{}
%\long\def\@enState[#1][#2][#3][#4][#5][#6]{\ensuremath{\tuple{#1, #2, #3, #4, #5, #6}}}
\long\def\@enState[#1][#2][#3][#4][#5][#6]{\ensuremath{\tuple{#1, #3, #4, #5, #6}}}
\newcommand{\enState}{\optparams{\@enState}{[\expr][\env][\store][\eventmap][\callinmap][\cont]}}

\newcommand{\@enSigState}{}
\long\def\@enSigState[#1][#2][#3]{\ensuremath{\tuple{#1, #2, #3}}}
\newcommand{\enSigState}{\optparams{\@enSigState}{[\absof{\trace}][\absof{\eventmap}][\absof{\callinmap}]}}


\newcommand{\Package}{\operatorname{pkg}}
\newcommand{\Msg}{\operatorname{msg}}

\newcommand{\fmttrans}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\enkwInit}{\fmttrans{init}}
\newcommand{\enkwEvt}{\fmttrans{evt}}
\newcommand{\enkwCb}{\fmttrans{cb}}
\newcommand{\enkwCi}{\fmttrans{ci}}
\newcommand{\enkwDis}{\fmttrans{dis}}
\newcommand{\enkwRet}{\fmttrans{ret}}
\newcommand{\enkwFin}{\fmttrans{fin}}
\newcommand{\enObs}[2]{\ensuremath{#1\;#2}}
\newcommand{\enInit}{\fmttrans{init}}
\newcommand{\enEvt}[1]{\ensuremath{\enkwEvt\;#1}}
\newcommand{\enCb}[1]{\ensuremath{\enkwCb\;#1}}
\newcommand{\enCi}[1]{\ensuremath{\enkwCi\;#1}}
\newcommand{\enDis}[1]{\ensuremath{\enkwDis\;#1}}
\newcommand{\enRet}[1]{\ensuremath{\enkwRet\;#1}}
\newcommand{\enFin}[1]{\ensuremath{\enkwFin\;#1}}
\newcommand{\silentTrans}{\ensuremath{\varepsilon}}

\newcommand{\@displaydiamond}{\scalebox{1.17}[0.87]{$\displaystyle\Diamond$}}
\newcommand{\@textdiamond}{\scalebox{1.17}[0.87]{$\textstyle\Diamond$}}
\newcommand{\@scriptdiamond}{\scalebox{1.15}[0.87]{$\scriptstyle\Diamond$}}
\newcommand{\@scriptscriptdiamond}{\scalebox{1.11}[0.87]{$\scriptscriptstyle\Diamond$}}

\newcommand{\diamondplus}{\mathbin{\mathchoice%
{\ooalign{\@displaydiamond\cr\hidewidth$\displaystyle+$}}%
{\ooalign{\@textdiamond\cr\hidewidth$\textstyle+$}}%
{\ooalign{\@scriptdiamond\cr\hidewidth$\scriptstyle+$}}%
{\ooalign{\@scriptscriptdiamond\cr\hidewidth$\scriptscriptstyle+$}}%
}}
\newcommand{\diamondminus}{\mathbin{\mathchoice%
{\ooalign{\@displaydiamond\cr\hidewidth$\displaystyle-$}}%
{\ooalign{\@textdiamond\cr\hidewidth$\textstyle-$}}%
{\ooalign{\@scriptdiamond\cr\hidewidth$\scriptstyle-$}}%
{\ooalign{\@scriptscriptdiamond\cr\hidewidth$\scriptscriptstyle-$}}%
}}

%\newcommand{\specArrow}{\mathord{\shortrightarrow}}
\newcommand{\specArrow}{\mathord{\rightarrow}}
\newcommand{\nspecArrow}{\mathord{\nrightarrow}}
%\newcommand{\specEnableOp}{\mathop{\diamondplus}}
\newcommand{\specEnableOp}{\mathop{\text{\relsize{-1}\enkwEvt}}}
%\newcommand{\specDisableOp}{\mathop{\diamondminus}}
\newcommand{\specDisableOp}{\mathop{\text{\relsize{-1}\enkwEvt}}}
%\newcommand{\specAllowOp}{\mathop{\boxplus}}
\newcommand{\specAllowOp}{\mathop{\text{\relsize{-1}\enkwCi}}}
%\newcommand{\specDisallowOp}{\mathop{\boxminus}}
\newcommand{\specDisallowOp}{\mathop{\text{\relsize{-1}\enkwCi}}}

\newcommand{\specEnable}[3][]{\ensuremath{#2 \specArrow_{#1} \specEnableOp #3}}
\newcommand{\specDisable}[3][]{\ensuremath{#2 \nspecArrow_{#1} \specDisableOp #3}}
\newcommand{\specAllow}[3][]{\ensuremath{#2 \specArrow_{#1} \specAllowOp #3}}
\newcommand{\specDisallow}[3][]{\ensuremath{#2 \nspecArrow_{#1} \specDisallowOp #3}}

\newcommand{\allSpecs}[4]{\ensuremath{{#3}_{\joinrel{#1}{#2}}(#4)}}
\newcommand{\allEnables}[1]{\allSpecs{\specArrow}{\specEnableOp}{}{#1}}
\newcommand{\allDisables}[1]{\allSpecs{\nspecArrow}{\specDisableOp}{}{#1}}
\newcommand{\allAllows}[1]{\allSpecs{\specArrow}{\specAllowOp}{}{#1}}
\newcommand{\allDisallows}[1]{\allSpecs{\nspecArrow}{\specDisallowOp}{}{#1}}
\newcommand{\allRules}[1]{\allSpecs{\dashrightarrow}{}{}{#1}}

\newcommand{\specPermit}[3][]{\ensuremath{#2 \specArrow_{#1} #3}}
\newcommand{\specForbid}[3][]{\ensuremath{#2 \nspecArrow_{#1} #3}}


\newcommand{\Trace}{\operatorname{tr}}
\newcommand{\Observe}{\operatorname{obs}}
\newcommand{\Args}{\operatorname{args}}
\newcommand{\EvtArgs}{\operatorname{xargs}}
\newcommand{\Partition}{\operatorname{parti}}
\newcommand{\Callbacks}{\operatorname{evtcbs}}
\newcommand{\Elimci}{\operatorname{elimci}}

\newcommand{\slicectx}{\ensuremath{\Delta}}
\newcommand{\traceslice}[3][\slicectx]{\ensuremath{#2 \upharpoonright_{#3}^{#1}}}

%%% Judgments
%\newcommand{\feasible}[2][\SpecSet]{ \ensuremath{\not\vdash_{#1} #2}}
\newcommand{\feasible}[2][\SpecSet]{\ensuremath{\entail[#1]{#2}{\bot}}}
\newcommand{\alarm}[2][\SpecSet]{\ensuremath{ \vdash^\epsilon_{#1} #2}} %%% should be deleted when we've fully converted to \notinit
%\newcommand{\notinit}[2][\SpecSet]{\ensuremath{\not\vdash^{\inittxtsub}_{#1} #2}}
\newcommand{\notinit}[2][\SpecSet]{\ensuremath{\vdash_{#1} #2\;\mathsf{excludesinit}}}
\newcommand{\entail}[3][\SpecSet]{ #2\vdash_{#1} #3 }
\newcommand{\empth}{\ensuremath{\mathtt{emp}}}
\newcommand{\quies}{\ensuremath{\texttt{fwk}}}
\newcommand{\applocterm}{\ensuremath{\texttt{app}}}
\newcommand{\errst}{\ensuremath{\mathtt{err}}}

%\newcommand{\ideq}[2]{\ensuremath{ #1 \stackrel{=}{\mathclap{\scriptscriptstyle{\text{id}}}} #2}}
%\newcommand{\idneq}[2]{\ensuremath{ #1 \stackrel{\neq}{\mathclap{\scriptscriptstyle{\text{id}}}} #2}}
%\newcommand{\ideq}[2]{\ensuremath{ \text{Ideq(}#1 , #2\text{)}}}
\newcommand{\unifysubst}{\vartheta}
\newcommand{\ideq}[2]{\ensuremath{#1 \simeq_{\unifysubst} #2}}
%\newcommand{\idneq}[2]{\ensuremath{ \neg\ideq{#1}{#2}}}
\newcommand{\idneq}[2]{\ensuremath{#1 \not\simeq #2}}

% matcher used for right hand side unrestricted
\newcommand{\directive}{\widetilde{\hist}}
\newcommand{\temporal}{\directive}
%\newcommand{\temporalfalse}{\fmtlogicconst{}{false}}
\newcommand{\temporaltrue}{\text{true}} %%% using this one for now because macro is not used consistently
\newcommand{\temporalfalse}{\text{false}} %%% using this one for now because macro is not used consistently

%Internal phi used in decision procedure
\newcommand{\phidec}{\ensuremath{\phi^{\mathtt{D}}}}

%negate only phi - syntactic restriction on possible 
\newcommand{\phineg}{\ensuremath{\directive^{\mathtt{U}}}}

\newcommand{\baks}[1]{\llbracket #1 \rrbracket_{\text{bk}}}
\newcommand{\baksover}[1]{\llbracket #1 \rrbracket_{\text{bk}}^{\#over}}
\newcommand{\baksunder}[1]{\llbracket #1 \rrbracket_{\text{bk}}^{\#under}}
\newcommand{\fwds}[1]{\llbracket #1 \rrbracket_{\text{fw}}}
\newcommand{\baksp}[1]{\baks{#1}^\text{a}}
\newcommand{\baksf}[1]{\baks{#1}^\text{f}} % trace abst filtered backward collecting semantics
\newcommand{\baksm}[1]{\llbracket #1 \rrbracket_{\text{b}}^m}
\newcommand{\jstep}[3][]{\ensuremath{#2 \rightarrow_{#1}^{\wfhist} #3}}
% \newcommand{\jstepstar}[3][]{\ensuremath{#2 \rightarrow_{#1}^{\wfhist\ast} #3}}
\newcommand{\jstepstar}[3][]{\ensuremath{#2 \rightarrow^{\ast} \mathrel{\substack{\wfhist\\ #1}} #3}}
\newcommand{\jstepins}[3]{\ensuremath{#1 \stackrel{\text{\normalsize$\longrightarrow$}}{\text{\scriptsize$#2$}} #3}}
\newcommand{\jstepinsstar}[3]{\ensuremath{#1 \stackrel{\text{\normalsize$\longrightarrow \ast$}}{\text{\scriptsize$#2$}} #3}}
\newcommand{\cbedge}[2]{[\enkwCb~#1]\hspace{-0.5em}\rightarrow #2}
\newcommand{\cfedgelefttail}{\mathord{-}\mkern-4mu\mathord{[}}
\newcommand{\cfedgerightarrow}{\mathord{]}\mkern-4mu\mathord{\shortrightarrow}}
\newcommand{\cfedge}[3]{#1\,\cfedgelefttail #2 \cfedgerightarrow\,#3}
\newcommand{\retedge}[2]{#1-\hspace{-0.6em} -\hspace{-0.22em} [#2]}
\newcommand{\rmstep}[3]{\ensuremath{ \langle #1 \rangle \stackrel{\text{\normalsize$\longrightarrow$}}{\text{\scriptsize$#2$}} \langle #3 \rangle }}
\newcommand{\rstep}[3][]{
 \ensuremath{ \langle #2 \rangle \longrightarrow_{#1} \langle #3 \rangle}
}
\newcommand{\rstepbad}[1]{
 \ensuremath{\langle #1 \rangle \longrightarrow \textbf{bad}}
}

\newcommand{\jcaption}[1]{\hfill\fbox{\normalsize$#1$}}
\newcommand{\wedgeover}[1]{\scalebox{1}{$\bigwedge$}_{#1}}

\newcommand{\wfhist}{\ensuremath{\Omega}}
\newcommand{\wfhistspec}{\ensuremath{\Omega_{\SpecSet}}}
%\newcommand{\wfhistjudge}[1]{\ensuremath{\mathcal{H}\llbracket #1 \rrbracket}}
\newcommand{\wfhistjudge}[1]{\ensuremath{#1 \in \wfhist}}

%% distilled semantics
\newcommand{\jeval}[4][\wfhist]{\ensuremath{\tuple{#2, #3} \Downarrow^{#1} #4}}
\newcommand{\jappeval}[3]{\ensuremath{\tuple{#1, #2} \Downarrow #3}}
\newcommand{\jseen}[2]{\ensuremath{#1 \vdash #2\;\mathsf{seen}}}
\newcommand{\jrealhist}[2][\wfhist]{\ensuremath{#1 \vdash #2}}
\newcommand{\jhoare}[3]{\ensuremath{\vdash \{ #1 \}\;#2\;\{ #3 \}}}
%\newcommand{\jtransok}[5][]{\ensuremath{#2 \vdash_{#1} \cfedge{#3}{#4}{#5}}}
\newcommand{\jtransok}[3][]{\ensuremath{#2 \vdash_{#1} #3}}
%\newcommand{\jmaywitness}[4][]{\ensuremath{#2 \vdash_{#1} #3 : #4}}
%% Caution: the following hardwires in \SpecSet, ignores #3
%\newcommand{\jmaywitness}[4][]{\ensuremath{#2 \vdash^{#1}_{\SpecSet} #4}}
\newcommand{\jmaywitness}[4][]{\ensuremath{#2 \vdash_{#1}^{\SpecSet} #4}}
%\newcommand{\jrefute}[3][]{\ensuremath{\not\vdash_{#1} #2 : #3}}
%\newcommand{\jrefute}[3][]{\ensuremath{\not\vdash_{#1} #3}}
%% Caution: the following hardwires in \SpecSet, ignores #2
%\newcommand{\jrefute}[3][]{\ensuremath{\vdash^{#1}_{\SpecSet} #3\;\mathsf{unreach}}}
\newcommand{\jrefute}[3][]{\ensuremath{\vdash_{#1}^{\SpecSet} #3\;\mathsf{unreach}}}
\newcommand{\semincluded}[2]{#1 \models #2}

\newcommand{\barmsg}{\bar{\msg}}
%%% Abstraction
\newcommand{\absmsg}{\absof{\msg}}
\newcommand{\absforce}{\absof{\imath}}
\newcommand{\initforce}{\mathsf{init}}

\newcommand{\abselem}{\ensuremath{\AIabselementfn}}
\newcommand{\absconc}{\ensuremath{\absof{\AIconcfn}}}
\newcommand{\conc}{\ensuremath{\AIconcfn}}
%% Caution: the following hardwires in \SpecSet
\newcommand{\inconc}[2]{\ensuremath{#1 \models_{\SpecSet} #2}}
\newcommand{\notinconc}[2]{\ensuremath{#1 \not\models_{\SpecSet} #2}}

\newcommand{\fmtlogicconst}[1]{\ensuremath{\mbox{\relscale{0.9}{$\mathsf{#1}$}}}}
\newcommand{\absappstore}{\absof{\appstore}}
\newcommand{\absappstate}{\absof{\appstate}}
\newcommand{\absmem}{\absof{\mem}}
\newcommand{\absmemFalse}{\bot}
\newcommand{\absmemOr}[2]{#1 \lor #2}
%% Caution: ignoring #4 for puredom
%\newcommand{\mkabsmem}[4]{\mkmem{#1}{#2}{#3} \cdot #4}
\newcommand{\mkabsmem}[4]{\mkmem{#1}{#2}{#3}}
%\newcommand{\mkshortabsmem}[3]{\ensuremath{\{#1 \textbf{:} #2 \cdot #3\}}}
\newcommand{\mkshortabsmem}[3]{\ensuremath{\{\,#1\colon #2 \cdot #3\,\}}}
\newcommand{\mkshorterabsmem}[2]{\ensuremath{\{\,#1\colon #2\,\}}}
\newcommand{\mkshortabsmemnostore}[2]{\ensuremath{\{\,#1\colon #2\,\}}}
\newcommand{\initabsappstate}{\absappstate_\inittxtsub}
\newcommand{\abspstate}{\absof{\pstate}}
\newcommand{\initabspstate}{\abspstate_\inittxtsub}
\newcommand{\invpstate}{\absof{\Sigma}}
\newcommand{\invemp}{\circ}
%% Caution: ignoring #2 for loc
%\newcommand{\invcons}[3]{#1, \mklocstate{#3}{#2}}
\newcommand{\invcons}[3]{#1, #3}
\newcommand{\absmsgstack}{\absof{\msgstack}}
\newcommand{\absmsgstackframe}{\absof{\msgstackframe}}
\newcommand{\absmsgstackemp}{\ltop}
\newcommand{\absmsgstackcons}[2]{#1 \mathbin{\bullet} #2}
\newcommand{\symval}{\hat{\var}}
\newcommand{\symvalseq}{\fmtseq{\symval}}
% \newcommand{\puredom}{\absof{\pi}}
\newcommand{\puredom}{????}
\newcommand{\puretrue}{\top}
\newcommand{\pureand}[2]{#1 \land #2}
\newcommand{\pureandseq}[2]{#1 \land \mathop{\mbox{\relscale{1.3}{$\land$}}}\fmtseq{#2}}
\newcommand{\pureseen}[1]{\fmtlogicconst{seen}(#1)}
%% Caution: ignoring #3 for puredom
%\newcommand{\mkabsappstate}[3]{\mkappstate{#1}{#2} \cdot #3}
\newcommand{\mkabsappstate}[3]{\mkappstate{#1}{#2}}
%% Caution: ignoring #5 for puredom
%\newcommand{\mkabspstate}[5]{\mkpstate{#1}{#2}{#3}{#4} \cdot #5}
\newcommand{\mkabspstate}[5]{\mkpstate{#1}{#2}{#3}{#4}}
\newcommand{\absappstoreTrue}{\ltop}
\newcommand{\absappstoreAnd}[2]{#1 \lsep #2}
\newcommand{\absappstorePtsto}[2]{#1 \ptsto #2}
\newcommand{\absappstoreSeq}[1]{\mathop{\Lsep}\fmtseq{#1}}
\newcommand{\absappstoreAndSeq}[2]{#1 \lsep \absappstoreSeq{#2}}

\newcommand{\valua}{\ensuremath{\theta}} %% todo - should be \assignment
\newcommand{\valuaemp}{\circ}
\newcommand{\valuaext}[3]{#1\extmap{#2}{#3}}
\newcommand{\valuaextseq}[3]{#1\fmtseq{\extmap{#2}{#3}}}
\newcommand{\withvalua}[2][\valua]{#2 \cdot #1}
\newcommand{\withvaluaind}[3][\valua]{#2 \cdot #1 \cdot #3}

\newcommand{\appop}{\operatorname{app}}
\newcommand{\appof}[1]{\appop(#1)}

\newcommand{\domop}{\operatorname{dom}}
\newcommand{\domof}[1]{\domop(#1)}

\newcommand{\locop}{\operatorname{loc}}
\newcommand{\locof}[1]{\locop(#1)}

%\def\arcr{\@arraycr}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Decision procedure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\toFOL}[1]{\ensuremath{\text{ToFoL(}#1\text{)}}}
\newcommand{\unsat}[1]{\ensuremath{\text{Unsat(}#1\text{)}}}
\newcommand{\sat}[1]{\ensuremath{\text{Sat(}#1\text{)}}}
\newcommand{\msgset}{\ensuremath{\SetName{Msg}}}
\newcommand{\addrset}{\ensuremath{\valset}}
\newcommand{\argset}{\ensuremath{\SetName{ArgIdx}}}
%\newcommand{\nameset}{\ensuremath{\SetName{ND}}}
\newcommand{\nameset}{\ensuremath{\SetName{MsgName}}}
\newcommand{\valset}{\ensuremath{\SetName{Val}}}

%uninterpreted indices in first order logic
\newcommand{\foli}{\ensuremath{\mathit{idx}}}
\newcommand{\folj}{\ensuremath{\mathit{u}_2}}
\newcommand{\folk}{\ensuremath{\mathit{u}_3}}

%TODO:rm once refactored
%\newcommand{\atEncode}[2]{\ensuremath{\text{E}_{#2} ( #1 )}}
\newcommand{\encodeRel}[3]{\ensuremath{\vdash_{#2} #1 \equiv #3}}
\newcommand{\toFOLRel}[2]{\ensuremath{\vdash #1 \equiv #2}}
\newcommand{\msgAtFolRel}[3]{\ensuremath{\vdash \text{MsgAtInd}(#1,#2) \equiv #3}}
\newcommand{\fol}{\ensuremath{\psi}}
%\stackrel{\text{\normalsize$\leadsto$}}{\text{\scriptsize#2}}
\newcommand{\dirEntailBot}[1]{#1\vdash \bot}
\newcommand{\empNotEntailDir}[1]{\notinit[]{#1}}
\newcommand{\dirEntailDir}[2]{#1 \vdash #2}
\newcommand{\histAxiomsFol}{\ensuremath{\fol_{\textrm{ax}}}}
\newcommand{\folEntailBot}[1]{\ensuremath{ \unsat{\histAxiomsFol \wedge #1}}}
\newcommand{\empNotEntailFol}[1]{\ensuremath{\unsat{\histAxiomsFol \wedge \fol \wedge \folLen = 0}}}
\newcommand{\folEntailFol}[2]{\ensuremath{\unsat{\histAxiomsFol \wedge #1 \wedge \forall \fv{#2}.~\neg #2}}}

%TODO: rm once refactored
%\newcommand{\updEncode}[2]{\ensuremath{\text{Q} ( #1, #2 ) }}

%\newcommand{\updRel}[3]{\ensuremath{#1 \vdash #2;#3}}
%\newcommand{\updRel}[3]{\ensuremath{\vdash #1 \equiv #2;#3}}
\newcommand{\updRel}[3]{\ensuremath{\vdash #1 \equiv #2 \fatsemi #3}}
%\newcommand{\instRel}[3]{\ensuremath{#1 \vdash_{#2} #3}}
\newcommand{\instRel}[3]{\ensuremath{#2, #1 \vdash #3}}

%rm once refactored
%\newcommand{\instEncode}[2]{\ensuremath{\text{I} ( #1, \SpecSet ) }}
%\newcommand{\instEncodeS}[2]{\ensuremath{\text{I} ( #1, #2 ) }}

%\newcommand{\msgequiv}[2]{\ensuremath{\text{Equiv(}#1,#2\text{)}}}
\newcommand{\msgequiv}[2]{\ensuremath{\text{Match(}#1,#2\text{)}}}
\newcommand{\folmsgequiv}[2]{\ensuremath{\text{EquivFoL(}#1,#2\text{)}}}
\newcommand{\folmsgnotequiv}[2]{\ensuremath{\neg\text{EquivFoL(}#1,#2\text{)}}}
\newcommand{\msgnotequiv}[2]{\ensuremath{\text{NotMatch(}#1,#2\text{)}}}
%\newcommand{\tracefn}{\ensuremath{\mathtt{tFN}}}
\newcommand{\tracefn}{\ensuremath{\fmtlogicconst{hist}}}
%\newcommand{\namefn}{\ensuremath{\mathtt{nFN}}}
\newcommand{\namefn}{\ensuremath{\fmtlogicconst{msgname}}}
%\newcommand{\argfn}{\ensuremath{\mathtt{aFN}}}
\newcommand{\argfn}{\ensuremath{\fmtlogicconst{msgargs}}}
%\newcommand{\unatset}{\ensuremath{\SetName{UNat}}}
\newcommand{\unatset}{\ensuremath{\SetName{HistIdx}}}
\newcommand{\boolset}{\ensuremath{\SetName{Bool}}}
\newcommand{\folLen}{\mathtt{len}}
\newcommand{\modDir}[2]{#1 \models #2}
\newcommand{\notModDir}[2]{#1 \not\models #2}
\newcommand{\modSpec}[2]{#1 \models #2}
\newcommand{\notModSpec}[2]{#1 \models #2}

\newcommand{\modeltriple}[3]{\ensuremath{#1\cdot#2\cdot#3}} % expect trace, assignment, position
\newcommand{\modeldouble}[2]{\ensuremath{#1\cdot#2}} % expect trace, assignment
\newcommand{\wellformed}[1]{\ensuremath{\text{Wf(}#1\text{)}}}
\newcommand{\wellformedU}[1]{\ensuremath{\text{Wf}^{\forall}\text{(}#1\text{)}}}

%highlight the fix in the overview example
\newcommand{\hlfix}{\footnotesize{\textit{ +fix}}}
\newcommand{\jmsgwithret}[4]{#1 = \jmsg{#2}{#3}{#4}}
\newcommand{\jmsg}[3]{#1\text{.}\codej{#2}\codej{(}#3\codej{)}}
\newcommand{\specci}[3]{\ensuremath{\enkwCi~#1\codej{.#2(}#3\codej{)}}}
\newcommand{\specciwithret}[4]{\ensuremath{\enkwCi~\ensuremath{#1}=\ensuremath{#2}\codej{.#3(}\ensuremath{#4}\codej{)}}}
\newcommand{\specstaticciwithret}[3]{\ensuremath{\enkwCi~\ensuremath{#1}=\codej{#2(}\ensuremath{#3}\codej{)}}}
\newcommand{\speccb}[3]{\ensuremath{\enkwCb\ #1 \codej{.}\codej{#2}\codej{(} #3 \codej{)}}}

\newcommand{\unsubmsgwidth}{0.22\linewidth}
\newsavebox{\SBoxUnsubMsgOne}
\begin{lrbox}{\SBoxUnsubMsgOne}
  \specci{\codej{s}}{unsubscribe}{} \hlfix
\end{lrbox}
\newsavebox{\SBoxUnsubMsg}
\begin{lrbox}{\SBoxUnsubMsg}
\lststopn\begin{lstdiffplus}[language=java,alsolanguage=exthighlighting,style=number,linewidth=\unsubmsgwidth,escapechar=|]
|\usebox{\SBoxUnsubMsgOne}|
\end{lstdiffplus}\lststartn
\end{lrbox}
\newcommand{\unsubmsghl}{\usebox{\SBoxUnsubMsg}}


\newsavebox{\SBoxPlayerFragmentTrace}
\begin{lrbox}{\SBoxPlayerFragmentTrace}\small
\begin{tabular}{l}
	\enkwCb\ \codej{@1.onCreate()}\\
	\enkwCi\ \codej{@2 = create(...)}\\
	\enkwCi\ \codej{@3 = @2.subscribe(@1)}\\
	\enkwCb\enkwRet\ \codej{@1.onCreate()}\\
	\enkwCb\ \codej{@1.onDestroy()}\\
	\enkwCi\ \codej{@3.unsubscribe()} ++\ \text{fix} \label{msg:fix}\\
	\enkwCb\enkwRet\ \codej{@1.onDestroy()}\\
	\enkwCb\ \codej{@1.call(...)} \text{assertion failure}\\
\end{tabular}
%\end{lstlisting}
\end{lrbox}
\newcommand{\ThePlayerFragmentTrace}{\scalebox{1}{\usebox{\SBoxPlayerFragmentTrace}}}
\newsavebox{\cfarrowbox}
\savebox{\cfarrowbox}{
\begin{tikzpicture}[node distance=0.5cm]
	\node(a)[draw=none]{};
	\node(b)[draw=none, right of=a]{};
	\path[-)] (a) edge (b);
\end{tikzpicture}
}
\newcommand{\cfarrow}{\hspace{-0.3cm}\usebox{\cfarrowbox}\hspace{-0.2cm}}
\newsavebox{\callarrowbox}
\savebox{\callarrowbox}{
\begin{tikzpicture}[node distance=0.5cm]
	\node(a)[draw=none]{};
	\node(b)[draw=none, right of=a]{};
	\path[{Straight Barb[left]}-{Straight Barb[left]}] (a) edge (b);
\end{tikzpicture}
}
\newcommand{\callarrow}{\hspace{-0.3cm}\usebox{\callarrowbox}\hspace{-0.2cm}}

%macros for overview abstract states
\newcommand{\ronepre}{\abstracecons{}{\speccb{\codej{f}}{call}{\codej{m}}}}
\newcommand{\rtwopre}{\abstracecons{}{\specci{\codej{s}}{unsubscribe}{}}}
\newcommand{\rthreepre}[3]{\abstracecons{}{\abstracecons{\specciwithret{#1}{#3}{subscribe}{#2}}{\speccb{#2}{onCreate}{}}}}
\newcommand{\lsvar}[1]{\codej{#1}}

% CBCFTL commands for syntax and semantic
\newcommand{\histlen}[1]{\ensuremath{\text{len}({#1})}}  % length of a message history
\newcommand{\lvar}[1]{\ensuremath{#1}}  % variable of the logic
\newcommand{\lvars}[1]{\ensuremath{\bar{#1}}} % Vector of variables in the logic
\newcommand{\lval}[1]{\ensuremath{#1}}  % variable of the logic
\newcommand{\lvals}[1]{\ensuremath{\bar{#1}}} % Vector of variables in the logic
\newcommand{\ldomain}{\ensuremath{\SetName{Val}}} % domain of the logic variables (values? to explain)
\newcommand{\assignment}{\ensuremath{\valua}}  % assignment
\newcommand{\fv}[1]{\ensuremath{\operatorname{fv}(#1)}} % Free variables for a formula

\newcommand{\ltmsg}{\ensuremath{\widetilde{\msg}}}
\newcommand{\ltrule}{\ensuremath{s}}
\newcommand{\ltpar}{\mathit{par}}

% Evaluation section macros

\newcommand{\benchmark}[2]{#1}
\newcommand{\apGa}{%
\benchmark{%
$\codej{getAct}^{[\reftr{spec:getActivityNull}]}$
}{1.4cm}%
}
\newcommand{\apEx}{%
\benchmark{%
$\codej{execute}^{[\reftr{spec:execute}]}$
}{1.6cm}%
}
\newcommand{\ymDi}{%
\benchmark{%
$\codej{dismiss}^{[\reftr{spec:dismiss}]}$
}{1.3cm}%
}
\newcommand{\cbFi}{%
\benchmark{%
$\codej{finish}^{\enkwNull}$
}{1.4cm}%
}
\newcommand{\synch}{%
  \benchmark{
  $\codej{subs}^{\enkwNull}$
  }{1.4cm}
}
\newcommand{\req}[1]{
  \textbf{RQ#1}
}

\newcommand{\thou}[1]{#1K}
\makeatother


==> program-logic.tex <==
\section{Abstract Application State and Abstract Messages}
\begin{figure}[H]
	\[
	\begin{array}{lrcll}
		\text{refutation state} & R \in \widehat{\StateSet} \ & ::= & (O,\, M,\, P)\\
    \text{abstract trace} & O & ::= & \epsilon \mid \absmsg \triangleright O\\
		\text{abstract store} & M & ::= & \top \mid \bot \mid {M}_1 \ast {M}_2 \\
		& & \mid & \absof{v_1}.f \mapsto \absof{v_2} \mid x \mapsto
    \absof{v} \\
		\text{pure constraints} & P & ::= & \enkwTrue \mid \enkwFalse \mid \absof{v}_1 = \absof{v}_2 \\
		& & \mid & \absof{v}_1 \not= \absof{v}_2  \mid P_1 \wedge P_2 \mid \absof{v}:\tau \\
		\text{symbolic varibles} & \hat{a}, \hat{b}, \hat{v} \in \absof{\SetName{Var}} \\
\text{abstract message} & \absmsg & ::= & \enkwCb\ n\ \absof{a}\\
    & & \mid & \absof{b} := \enkwCi\ n\ \absof{a}\\
    & & \mid &\absof{b} :=\enkwCb\enkwRet\ n\ \absof{a}\\
\text{concretization} & \langle \omega, \rho \rangle \in \gamma(R,\SpecSet{} )\\
	\end{array}
	\]
	\caption{The refutation state captures an abstraction of the application heap, $M$, and a list of abstractions representing sets of traces that may reach the expectation, $O$.  The heap abstraction is represented by a separation logic formula. Symbolic variables, $\hat{x}$, represent a single concrete value at runtime that is existentially quantified for the current refutation state. Concretization takes an abstract state and a spec set and returns a set of traces and heaps.}
\end{figure}

%%  \newcommand{\largeast}{\ \underset{i}{\text{\Large{\Large$\ast$}}}\ }
%%  \begin{figure}[H]
%%  \small{
%%    \[
%%    \begin{array}{l}
%%      \boxed{\mathit{app}, \SpecSet \vdash \{R_{\text{pre}}\} t \{R_{\text{post}}\}:\absof{\msg}}\\\\
%%      \infer[a-callback invoke]{\absmsg = \enkwCb\ n\ \absof{a} \\ \cfedge{\ell'}{n}{\ell} \in \mathit{app} \\ \absmsg' = \absof{b} := \enkwCb\enkwRet\ n\ \absof{a} \\ (n,\tau \rightarrow \tau') \in \SetName{Interface} \\ P' = P \wedge \absof{a}:\tau} {
%%        \mathit{app},\SpecSet\vdash \{\absof{\rho}\wedge P', \epsilon\}\cfedge{\ell'}{n}{\ell} \{\absof{\rho} \ast \codej{p1} \mapsto \absof{a} \wedge P, \ell;\absmsg';\epsilon\}:\absmsg
%%      }\\\\
%%      \infer[a-callback return]{ 
%%        \absof{m} = \absof{a} := \enkwCb\enkwRet\ n\ \absof{b} \\ \text{fresh}(\absof{a},\absof{b}) \\ \cfedge{\ell'}{\enkwRet\ x}{\ell} \in \mathit{app} \\ (n,\tau \rightarrow \tau') \in \SetName{Interface}\\ P' = P \wedge \absof{a} : \tau' \wedge \absof{b}:\tau
%%        }{
%%        \mathit{app},\SpecSet \vdash \{\absof{\rho} \ast x \mapsto \absof{a} \ast \codej{p1} \mapsto \absof{b} \wedge P', \ell';\absmsg;\epsilon\} \cfedge{\ell'}{\enkwRet\ x}{\ell} \{\absof{\rho}\wedge P, \epsilon\}:\absmsg
%%      }\\\\
%%      \infer[a-callin invoke]{\absmsg = \enkwCi\ n\ \absof{a} \\ \cfedge{\ell'}{x := \enkwInvoke\ n\ y}{\ell} \in \mathit{app} \\ \absmsg' = \absof{b} := \enkwCi\enkwRet\ n\ \absof{a} \\ (n,\tau \rightarrow \tau') \in \SetName{Interface} \\ P' = P \wedge \absof{a}:\tau }{
%%        \mathit{app},\SpecSet \vdash  \{\absof{\rho} \ast y \mapsto \absof{b} \wedge P',\ \ell';\absof{k}'\} \cfedge{\ell'}{x := \enkwInvoke\ n\ y}{\ell} \{\absof{\rho} \ast y \mapsto \absof{b} \wedge P,\ \absof{m}';\ell';\absof{k}\}:\absmsg
%%      }\\\\
%%      \infer[a-callin return]{ \absmsg = \absof{a} := \enkwCi\enkwRet\ n\ \absof{b} \\ \cfedge{\ell'}{x:=\enkwInvoke\ n\ y}{\ell} \in \mathit{app} \\ (n,\tau \rightarrow \tau') \in \SetName{Interface} \\ P' = P \wedge \absof{a}:\tau' }{
%%        \mathit{app},\SpecSet \vdash  \{\absof{\rho} \ast y \mapsto \absof{b} \wedge P',\ \absof{m};\ell';\absof{k}'\} \cfedge{\ell'}{x := \enkwInvoke\ n\ y}{\ell} \{\absof{\rho} \ast x \mapsto \absof{a} \ast y \mapsto \absof{b} \wedge P,\ \ell;\absof{k}\}:\absmsg
%%      }\\\\
%%    \end{array}
%%    \]
%%    \[
%%    \begin{array}{l r}
%%      \boxed{\mathit{app}, \SpecSet \vdash \{R_{\text{pre}}\} t \{R_{\text{post}}\}}\\
%%      \infer[skip]{ }{\vdash \{\text{any}\wedge P,\ \ell';\absof{k}\}\cfedge{\ell'}{c}{\ell} \{\text{any} \wedge P,\ \ell;\absof{k}\} } &
%%      \infer[new]{ \absof{v} \notin \absof{\rho} \\ \absof{p}:\tau } {
%%        \vdash \{\absof{\rho} \wedge P,\ \ell';\absof{k}\} \cfedge{\ell'}{x := \enkwNew\ \tau}{\ell}\{\absof{\rho} \ast x \mapsto \absof{v} \wedge P,\ \ell;\absof{k} \}
%%      }\\\\
%%    \end{array}
%%    \]
%%    \[
%%    \begin{array}{l r}
%%      \infer[frame]{ \vdash \{\absof{\rho}' \wedge P',\ \absof{k}'\}t\{\absof{\rho} \wedge P',\ \absof{k}\} \\ \text{t cannot modify }\absof{\rho}_2 }{
%%        \vdash \{ (\absof{\rho}_2 \ast \absof{\rho}') \wedge P,\ \absof{k}' \} t \{ (\absof{\rho}_2 \ast \absof{\rho}) \wedge P ,\ \absof{k}\}
%%      }\\\\
%%      \infer[assign]{ }{
%%      \vdash \{y \mapsto \absof{v} \wedge P,\ \ell';\absof{k}\} \cfedge{\ell'}{x := y}{\ell} \{x \mapsto \absof{v} \wedge P,\ \ell;\absof{k} \}
%%      }\\\\
%%      \infer[read]{ }{
%%      \vdash \{\exists \absof{a}.y \mapsto \absof{v} \wedge P,\ \ell';\absof{k}\} \cfedge{\ell'}{x := y.f}{\ell} \{x \mapsto \absof{v} \wedge P,\  \ell;\absof{k}\}
%%      }\\\\
%%      \infer[write-alias]{P' = P \wedge \forall i. \absof{a} \not= \absof{b}_i \\ \absof{\rho} = (\largeast \absof{b}_i.f \mapsto \absof{c}_i )}{
%%      \vdash \{\absof{\rho} \ast \exists \absof{a}. x \mapsto \absof{a} \ast y \mapsto \absof{v} \wedge P',\ \ell';\absof{k} \}\cfedge{\ell'}{x.f := y}{\ell}\{\absof{a}.f \mapsto \absof{v} \ast \absof{\rho} \wedge P,\ \ell;\absof{k} \}
%%      }\\\\
%%      \infer[write-no-alias]{P' = P \wedge \forall i. \absof{a} \not= \absof{b}_i \\ \absof{\rho} = (\largeast \absof{b}_i.f \mapsto \absof{c}_i ) }{
%%        \vdash \{\absof{\rho} \ast \exists \absof{a} . x \mapsto \absof{a} \wedge P',\ \ell';\absof{k} \} \cfedge{\ell'}{x.f := y}{\ell} \{\absof{\rho} \wedge P,\ \ell;\absof{k}\}
%%      }
%%    \end{array}
%%    \]
%%    }
%%  %	\[
%%  %	\begin{array}{rcl}
%%  %	\text{prepend}(\psi;O, \absmsg) & \defeq & 	\text{prepend}(\psi,\absmsg);\text{prepend}(O,\absmsg)\\
%%  %	\text{prepend}(\epsilon, \absmsg)& \defeq & \epsilon\\
%%  %	\text{prepend}(\psi \triangleright \absmsg_2, \absmsg_1) & \defeq & \text{prepend}(\psi, \absmsg_1) \triangleright \absmsg_2\\
%%  %	\text{prepend}(\psi_1 \wedge \psi_2, \absmsg) & \defeq & \text{prepend}(\psi_1, \absmsg) \wedge \text{prepend}(\psi_2, \absmsg)\\
%%  %	\text{prepend}(\niDir{\absmsg_1}{\absmsg_2}, \absmsg) & \defeq & \niDir{\absmsg_1}{\absmsg_2} \triangleright \absmsg \\
%%  %	\text{prepend}(\iDir{\absmsg_1}, \absmsg) & \defeq & \iDir{\absmsg_1} \triangleright \absmsg \\
%%  %	\end{array}
%%  %	\]
%%    \caption{\TODO{$\vdash \{R\}t\{R\}$ modifies thresher's definition to track the stack and use multiple states to represent disjunction rather than including $\vee$ in the refutation state. Cite here.}Abstract semantics of computing the refutation state of a predecessor location based on the current location's refutation state. The helper function pop checks for a valid abstract stack and returns the new abstract stack, push adds a callback and location to the abstract stack. \TODO{should we use types, $\tau$, to indicate possible aliasing? If not we should remove them from formalism.}}
%%    \label{fig:absSemantics}
%%  \end{figure}


%-----------------------------------------------
%     STATIC SEMANTICS
%-----------------------------------------------
\input{staticsem}




==> staticsem_mem.tex <==

% ----------------------------------------------------------- %
%             TRACE + HEAP REASONING
% ----------------------------------------------------------- %
\ignore{
\begin{figure}[H] % TODO: switch back to "ht" after structure is fixed.

%
  \fbox {\(\SpecSet \vdash \{R'\} ~c~ \{R\} \)}
%
\bigskip

\begin{minipage}{2.25in}
\begin{mathpar}
\begin{array}{c}
  \infer[a-callback witness]
  {
    %n:\,\{x:\tau\} \rightarrow \tau'\\
%    \mathtt{SAT}(\enkwCb\ n\ \absof{a};O,\SpecSet, M, P)\\
	\SpecSet, \epsilon,\text{emp} \models \ll \enkwCb\ n\ \absof{a}\triangleright O, M, P \gg
  } 
  {
			\SpecSet\vdash 
      \{\enkwCb\ n\ \absof{a} \triangleright O,\, \top,\, \enkwTrue\} 
        ~n~ 
      \{O,\, M,\, P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
%
\begin{minipage}{2.25in}
\begin{mathpar}
\begin{array}{c}
  \infer[a-callback invoke]
  {
    n:\,\{x:\tau\} \rightarrow \tau'\\
    %\mathtt{UNSAT}(O,\SpecSet, \rho, P)
  } 
  {
			\SpecSet\vdash 
      \{\enkwCb\ n\ \absof{a}\triangleright O,\, M,\, P\} 
        ~n~ 
      \{O,\, M * x\mapsto \absof{a},\, P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip

%
\begin{minipage}{\linewidth}
\begin{mathpar}
\begin{array}{c}
  \infer[a-callback return]
  {
    \mathtt{fresh}(\absof{a},\absof{b})\\
    n:\,\{x:\tau\} \rightarrow \tau'\\
  } 
  {
			\SpecSet\vdash 
      \{\absof{a} := \enkwCb\enkwRet\ n\ \absof{b}\triangleright O,\, 
        M * y\mapsto \absof{a} * x\mapsto \absof{b},\, 
        P \wedge \absof{a}:\tau' \wedge \absof{b}:\tau\} 
        ~\enkwRet\ n\ y~ 
      \{O,\, M,\, P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip

%
\begin{minipage}{\linewidth}
\begin{mathpar}
\begin{array}{c}
  \infer[a-callin invoke]
  {
    n:\,\{x:\tau\} \rightarrow \tau'\\
  } 
  {
			\SpecSet\vdash 
      \{\absof{a} := \enkwCi\ n\ \absof{b} \triangleright O,\, 
        M * y\mapsto \absof{b},\, P \wedge \absof{b}:\tau \wedge
        \absof{a}:\tau'\} 
        ~x :=  \enkwInvoke\ n\ y~ 
      \{O,\, M*x\mapsto \absof{a} * y \mapsto \absof{b},\, P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip

%
\begin{minipage}{2.25in}
\begin{mathpar}
\begin{array}{c}
  \infer[a-skip refute]
  {
%    \mathtt{UNSAT}(\omega;O,\, S,\, M,\, P)\\
     \not\exists \omega, \rho \text{\ .\ } \SpecSet, \omega,\rho \models \ll O,M,P \gg
  } 
  {
			\SpecSet\vdash 
      \{O,\, \bot,\, \enkwFalse\} 
        ~\texttt{\bf skip}~ 
      \{O,\, M,\, P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip

%
\begin{minipage}{2.25in}
\begin{mathpar}
\begin{array}{c}
  \infer[a-abstraction]
  {
      \vdash \{R_2'\} c \{R_2\} \\
      R_2', \SpecSet \models R_1', \SpecSet \\ 
      R_1, \SpecSet \models R_2, \SpecSet \\
  } 
  {
			\SpecSet\vdash 
      \{R_1'\} 
        ~c~ 
      \{R_1\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
%
\begin{minipage}{2.25in}
\begin{mathpar}
\begin{array}{c}
  \infer[a-com lift]
  {
    \{M',\, P'\} ~c~ \{M,\, P\}
  } 
  {
			\SpecSet\vdash 
      \{O,\, M',\, P'\} ~c~ \{O,\, M,\, P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip
\caption{Combined trace and memory reasoning.}
%\caption{Combined Trace and Heap Reasoning. $R_1,\SpecSet \models R_2,\SpecSet$ iff $\forall \langle \omega , \rho \rangle \in \gamma(R_2,\SpecSet) . \langle \omega, \rho \rangle \in \gamma(R_1,\SpecSet)$. Decision procedures encoded in SAT can be found in figure \ref{fig:sat}. (\TODO{$\text{emp}$ represents the empty/initial concrete heap})}
\label{fig:staticsem-1}
\end{figure}
}
% ----------------------------------------------------------- %
%             HEAP REASONING
% ----------------------------------------------------------- %


\begin{figure}[H] %TODO: switch back to "ht" after structure is fixed
%
  \fbox {\(\{M', P\} ~c~ \{M,P\} \)}
%
\bigskip

%
\begin{minipage}{2.5in}
\begin{mathpar}
\begin{array}{c}
  \infer[new]
  {
    \absof{v} \not\in M\\
    \absof{v} \not\in P\\
  } 
  {
    \{M,\, P \wedge \absof{v}:T\} 
        ~x :=  \enkwNew\ T()~ 
    \{M*x\mapsto \absof{v},\, P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
%
\begin{minipage}{2.25in}
\begin{mathpar}
\begin{array}{c}
  \infer[new refute]
  {
    \absof{v} \in M \vee
    \absof{v} \in P\\
  } 
  {
    \{\bot,\, \enkwFalse\} 
        ~x :=  \enkwNew\ T()~ 
    \{M*x\mapsto \absof{v},\, P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip

%
\begin{minipage}{\linewidth}
\begin{mathpar}
\begin{array}{c}
  \infer[assign]
  {
  } 
  {
    \{M * y\mapsto \absof{v_2},\, 
      P \wedge \absof{v_2} = \absof{v_1}\} 
        ~x :=  y~ 
    \{M*x\mapsto \absof{v_1} * y\mapsto \absof{v_2},\, P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip

%
\begin{minipage}{\linewidth}
\begin{mathpar}
\begin{array}{c}
  \infer[read]
  {
  } 
  {
    \{M * y\mapsto \absof{v_2} * \absof{v_2}.f \mapsto \absof{v_3},\, 
      P \wedge \absof{v_1} = \absof{v_3}\} 
        ~x :=  y.f~ 
    \{M * x\mapsto \absof{v_1} * y\mapsto \absof{v_2} * \absof{v_2}.f \mapsto \absof{v_3},\, 
      P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip

%
\begin{minipage}{\linewidth}
\begin{mathpar}
\begin{array}{c}
  \infer[write]
  {
  } 
  {
    \{M * x\mapsto \absof{v_1} * y \mapsto \absof{v_3},\, 
      P \wedge \absof{v_2} = \absof{v_3}\} 
        ~x.f :=  y~ 
    \{M * x\mapsto \absof{v_1} * \absof{v_1}.f \mapsto \absof{v_2} * 
        y \mapsto \absof{v_3},\, 
      P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip

%
\begin{minipage}{\linewidth}
\begin{mathpar}
\begin{array}{c}
  \infer[assume]
  {
  } 
  {
    \{M * x\mapsto \absof{v_1} * y \mapsto \absof{v_2},\, 
      P \wedge \Phi(\absof{v_1},\absof{v_2})\} 
        ~\enkwAssume\ \Phi(x,y)~ 
    \{M * x\mapsto \absof{v_1} *  y \mapsto \absof{v_2},\, 
      P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip

%
\begin{minipage}{2.25in}
\begin{mathpar}
\begin{array}{c}
  \infer[materialize]
  {
    x \not\in M \\
    \mathtt{fresh}(\absof{v})\\
  } 
  {
    \{M * x\mapsto \absof{v},\, P \} 
        ~ \texttt{\bf skip}~ 
    \{M ,\, P\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip


\caption{Heap Reasoning}
\label{fig:staticsem-2}
\end{figure}
%




==> staticsem_trace.tex <==

% ----------------------------------------------------------- %
%             TRACE + HEAP REASONING
% ----------------------------------------------------------- %
\begin{figure} % TODO: switch back to "ht" after structure is fixed.
\begin{minipage}{9cm}
\[
\begin{array}{lrcll}
	\text{lifted commands} & c_i & \bnfdef & \enkwCb~n~\bar{x} \bnfalt \enkwRet~n \bnfalt s\\
	\text{abstract traces} & \abstrace & ::= & \abstracebase \mid \abstrace \triangleright \absof{m}\\
	\text{abstract store} & \absof{\rho} & \bnfdef & \epsilon \bnfalt \absof{\rho}[x \mapsto \absof{v}]\\
	\text{abstract stack} & \absof{\stack} & \bnfdef & \cdot \bnfalt \absmsg~\absof{\rho}\\
	\text{abstract heap} & \absof{\sigma} & \bnfdef & \mathtt{any} \mid ...\\
	\text{refutation state} & \refstate \in \absof{\SetName{State}} & \bnfdef & \{ \abstrace, \absof{\sigma}, \absof{\stack} \}\\
	& & \bnfalt & \refstate \vee \refstate' \bnfalt \bot \bnfalt \top\\
%	\text{state set} & A \in \absof{\SetName{State}} & \bnfdef & \bot \mid A \vee \refstate \\
	%TODO: following should probably be added to appendix for mem abstraction
%		\text{abstract memories} & M & \bnfdef & \mathtt{any} \mid x \mapsto \absof{v} \mid M \ast M' \mid ...\\
%	\text{memories} & M & ::= & any \mid \absof{v}_1.f \mapsto \absof{v}_2 \mid ...\\
%	\text{pure formula} & P & ::= & true \mid \wedge \mid \vee \mid \absof{v}_1 = \absof{v}_2 \mid \neg P \mid ...\\
%	\text{abstract messages} & \absmsg & \bnfdef & ...\\%n\ \absof{v}\\
\text{abstract message} & \absmsg & \bnfdef & \absof{v}' := \enkwCi~n~\bar{\absof{v}} \bnfalt \enkwCb~n~\bar{\absof{v}} \\
& & \bnfalt & \enkwCb\enkwRet~n~\bar{\absof{v}}\\
	\text{abstract values} & \absof{v} & \bnfdef & \absof{a} \bnfalt \absof{b} \bnfalt ... \\
\text{invariant map} & I & : & \SetName{Loc} \rightarrow \absof{\SetName{State}}
%	\text{concretization} & \omega & \in & \gamma(\abstrace)\\
\end{array}
\]
\end{minipage}%
\begin{minipage}{5cm}
\begin{center}
\fbox{\(I \vdash \cfedge{\mathit{cl}}{c_i}{\mathit{cl'}} \)}
\end{center}
\bigskip
\begin{mathpar}
	\infer[A-Transition]{\vdash \{\refstate'\} ~c_i~ \{\refstate\} \\ \entail[]{R'}{I(\mathit{cl})} \\ \entail[]{I(\mathit{cl}')}{R}  }{
		I \vdash \cfedge{\mathit{cl}}{c_i}{\mathit{cl'}}
	}
\end{mathpar}
\end{minipage}
%
  \fbox {\(\vdash \{\refstate'\} ~c_i~ \{\refstate\} \)}
%
\bigskip
%

\begin{minipage}{10cm}
\infer[a-query-start]
{
%  	\mathtt{fresh}(\bar{\absof{a}})\\ % Don't need fresh since post state is empty
  	n~\text{is}~\enkwCb~\text{containing}~\enkwAssert
} 
{
			\vdash 
      \{ \abstracebase,\, \mathtt{any},\, \enkwCb~n~\bar{\absof{a}}\} 
        ~\enkwAssert~ 
      \{ \bot\}%
}
\end{minipage}%
\begin{minipage}{10cm}
\infer[a-callback-alarm]
{
	\alarm[]{\abstrace \triangleright \enkwCb~n~\absof{a}} \\ 
	\absmsg = \enkwCb~n~\bar{\absof{a}}
} 
{
			\vdash 
      \{ \top\} 
        ~\enkwCb~n~\bar{x}~ 
      \{\abstrace,\, \absof{\sigma}, \absof{m}[\bar{x} \mapsto \bar{\absof{a}}]\}
}
\end{minipage}

%
%

\begin{minipage}{2.25in}
  \infer[a-callback-invoke]
  {
%    n:\,\{x:\tau\} \rightarrow \tau'\\
    %\mathtt{UNSAT}(O,\SpecSet, \rho, P)
    \absmsg = \enkwCb~n~\bar{\absof{a}}
  } 
  {
			\vdash 
      \{\abstrace \triangleright \enkwCb\ n\ \bar{\absof{a}},\, \absof{\sigma},\, \cdot\} 
        ~\enkwCb~n~\bar{x}~ 
      \{\abstrace,\, \absof{\sigma},\, \absmsg [\bar{x}\mapsto \bar{\absof{a}}]\}
	}
\end{minipage}%
\begin{minipage}{2.25in}
\begin{mathpar}
\begin{array}{c}
  \infer[a-callback-return]
  {
    \mathtt{fresh}(\bar{\absof{a}})\\ \absmsg = \enkwCb~n~\bar{\absof{a}}
        %\mathtt{quiescent}(\abstrace)\\
%    n:\,\{x:\tau\} \rightarrow \tau'\\
  } 
  {
			\vdash 
      \{\abstrace \triangleright \enkwCb\enkwRet\ n\ \bar{\absof{a}},\, 
        \absof{\sigma},\, \absmsg [\bar{x} \mapsto \bar{\absof{a}}] 
%        P \wedge \absof{a}:\tau' \wedge \absof{b}:\tau
        \} 
        ~\enkwRet\ n~ 
      \{\abstrace,\, \absof{\sigma},\, \cdot\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip

%
\begin{minipage}{\linewidth}
\begin{mathpar}
\begin{array}{c}
  \infer[a-callin-invoke]
  {
  	\absmsg = \absof{a} := \enkwCi~n~\bar{\absof{b}} \\ \absof{\stack} = \absof{\stack}'[\bar{y} \mapsto \bar{\absof{b}}]
%    n:\,\{x:\tau\} \rightarrow \tau'\\
  } 
  {
			\vdash 
      \{\abstrace \triangleright \absmsg\, , 
        \absof{\sigma},\, \absof{\stack}\} 
        ~x :=  \enkwInvoke~\enkwCi~n\ \bar{y}~ 
      \{\abstrace,\, \absof{\sigma},\, \absof{\stack}[x\mapsto \absof{a}]\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
\bigskip

\begin{tabular}{l r}
%
\begin{minipage}{1.5in}
\begin{mathpar}
\begin{array}{c}
  \infer[a-callback-refute]
  {
     \feasible[]{\abstrace\triangleright\enkwCb~n~\bar{\absof{a}}}\\
  } 
  {
			\vdash 
      \{\bot\} 
        ~\enkwCb~n~\bar{x}~ 
      \{\abstrace,\, \absof{\sigma},\, \absof{k}[\bar{x} \mapsto \bar{\absof{a}}]\}
	}
\end{array}
\end{mathpar}
\end{minipage}
%
%\bigskip
&
%
\begin{minipage}{2.25in}
\begin{mathpar}
\begin{array}{c}
  \infer[a-com-lift]
  {
    \{\absof{\sigma}'\} ~c~ \{\absof{\sigma}\}
  } 
  {
			\vdash 
      \{\abstrace,\, \absof{\sigma}',\, \absof{k}\} ~c~ \{\abstrace,\, \absof{\sigma},\, \absof{k}\}
	}
\end{array}
\end{mathpar}
\end{minipage}
\end{tabular}
%
%
%\begin{minipage}{1.5in}
%\begin{mathpar}
%\begin{array}{c}
%  \infer[a-abstraction]
%  {
%      \vdash \{\refstate_2'\} c \{\refstate_2\} \\
%      \refstate_2' \vdash \refstate_1' \\ 
%      \refstate_1  \vdash \refstate_2 \\
%  } 
%  {
%			\vdash 
%      \{\refstate_1'\} 
%        ~c~ 
%      \{\refstate_1\}
%	}
%\end{array}
%\end{mathpar}
%\end{minipage}
%
\bigskip
\caption{Static semantics over application commands that emit observable messages.  We use a circumflex on a concrete metavariable to denote the abstract version (e.g. the metavariable $\omega$ represents a concrete trace whereas $\absof{\omega}$ represents an abstract trace).  Similar to concrete metavariables, we use a bar to represent a vector of abstract values (e.g. $\bar{\absof{a}}$ means a comma-separated list of abstract values).  }
%\caption{Combined Trace and Heap Reasoning. $R_1,\SpecSet \models R_2,\SpecSet$ iff $\forall \langle \omega , \rho \rangle \in \gamma(R_2,\SpecSet) . \langle \omega, \rho \rangle \in \gamma(R_1,\SpecSet)$. Decision procedures encoded in SAT can be found in figure \ref{fig:sat}. (\TODO{$\text{emp}$ represents the empty/initial concrete heap})}
\label{fig:staticsem-1}
\end{figure}

